MillenniumDB: A Persistent, Open-Source, Graph Database

In this systems paper, we present MillenniumDB: a novel graph database engine that is modular, persistent, and open source. MillenniumDB is based on a graph data model, which we call domain graphs, that provides a simple abstraction upon which a variety of popular graph models can be supported. The engine itself is founded on a combination of tried and tested techniques from relational data management, state-of-the-art algorithms for worst-case-optimal joins, as well as graph-specific algorithms for evaluating path queries. In this paper, we present the main design principles underlying MillenniumDB, describing the abstract graph model and query semantics supported, the concrete data model and query syntax implemented, as well as the storage, indexing, query planning and query evaluation techniques used. We evaluate MillenniumDB over real-world data and queries from the Wikidata knowledge graph, where we find that it outperforms other popular persistent graph database engines (including both enterprise and open source alternatives) that support similar query features.

==> sections/data-ah.tex <==
%!TEX root = ../main.tex

We first discuss popular graph data models and their limitations. We then introduce the graph data model we have chosen. %We will use the Wikidata knowledge graph~\cite{VrandecicK14} as a real-world use-case to exemplify and motivate our proposed model, and to illustrate its benefits vs.\ similar models that are popular in practice.

\subsection{Graph Data Models}

One of the simplest models used for representing knowledge graphs is based on \textit{directed labelled graphs}, which consist of a set of nodes and edges such that every edge relates a pair of nodes. An edge is graphically represented as \gedge[arrin][0.6cm]{$a$}{$b$}{$c$}, where $a$ is called the source node, $b$ the edge label, and $c$ the target node. Such graphs are the basis of the RDF data model~\cite{CyganiakWL14}, where the source node, edge label and target node are called \textit{subject}, \textit{predicate} and \textit{object}, respectively. In the context of knowledge graphs, nodes are used to represent entities and edges represent binary relations. For example, with the edge \gedge[arrin][1.8cm]{Michelle Bachelet}{position held}{President of Chile}, we can state that Michelle Bachelet was (or is) the president of Chile.
%A popular concrete model based on \textit{directed edge-labelled graphs} is the RDF model~\cite{CyganiakWL14}. 

However, directed labelled graphs are sometimes \textit{too} simple. While they elegantly represent binary relations, they are cumbersome when representing higher arity relations. Take, for example, the statements from the Wikidata knowledge graph~\cite{VrandecicK14} illustrated in Figure~\ref{fig:mb}. We see that the statements encode the same binary relation, but it is now associated with nested \textit{qualifiers} that provide additional information: in this case a start date, and end date, who replaced her, and whom she was replaced by. We also see that the same binary relation is expressed twice, indicating two distinct periods when she held the position. Representing statements like this in a directed labelled graph requires some form of \textit{reification} to decompose $n$-ary relations into binary relations~\cite{HernandezHK15}. For example, Figure~\ref{fig:delg} shows a graph where $e_1$ and $e_2$ are nodes representing $n$-ary relationships. The reification is given by the use of the edges labelled as \texttt{source}, \texttt{label} and \texttt{target}. For simplicity, we use human-readable nodes and labels, where in practice, a node \gnode{Sebastián Piñera} will rather be given as the identifier \gnode{Q306}, and an edge label \texttt{replaces} will rather be given as \texttt{P155}.

\newcommand{\wid}[1]{{\color{gray}~[#1]}} % format Wikidata IDs

\begin{figure}[tb]
\centering
{\sf
\begin{tabular}{l}
\large\textbf{Michelle Bachelet\wid{Q320}}\\[1ex]
\large\qquad position held\wid{P39} \quad President of Chile\wid{Q466956}\\
\qquad \qquad 
{\begin{tabular}{l@{\qquad~~}l}
start date \wid{P580} & 2014-03-11\\
end date \wid{P582} 	& 2018-03-11\\
replaces\wid{P155}	& Sebastián Piñera\wid{Q306}\\
replaced by\wid{P156} & Sebastián Piñera\wid{Q306}\\
\end{tabular}}\\
\\[-1ex]
\large\qquad position held\wid{P39} \quad President of Chile\wid{Q466956}\\
\qquad \qquad {\begin{tabular}{l@{\qquad~~}l}
start date \wid{P580} & 2006-03-11\\
end date \wid{P582} & 2010-03-11\\
replaces\wid{P155} & Ricardo Lagos\wid{Q331}\\
replaced by\wid{P156} & Sebastián Piñera\wid{Q306}\\
\end{tabular}}
\end{tabular}
}
\caption{Wikidata statement group for Michelle Bachelet \label{fig:mb}}
\end{figure}


%\begin{figure}[t]
%\centering
%\includegraphics[width=8.5cm]{./images/digraph.png}
%\caption{Directed edge-labelled graph reifying the statements of Figure~\ref{fig:mb} \label{fig:delg}}
%\end{figure}


\begin{figure}[t]
\setlength{\vgap}{0.45cm}
\setlength{\hgap}{2.5cm}
\centering
\begin{tikzpicture}
\node[iri] (e1) {$e_1$};

\node[iri,right=\hgap of e1] (pe1) {position held}
  edge[arrin] node[lab] {label} (e1);
  
\node[iri,above=\vgap of pe1] (se1) {Michelle Bachelet}
  edge[arrin] node[lab] {source} (e1);
  
\node[iri,below=\vgap of pe1] (oe1) {President of Chile}
  edge[arrin] node[lab] {target} (e1);
 
\node[iri,above=\vgap of se1] (sp) {Sebastian Piñera}
  edge[arrin] node[lab] {replaced by} (e1)
  edge[arrin,bend right=19] node[lab,pos=0.45] {replaces} (e1);
  
\node[iri,right=\hgap of pe1] (e2) {$e_2$}
  edge[arrout] node[lab] {label} (pe1)
  edge[arrout] node[lab] {source} (se1)
  edge[arrout] node[lab] {target} (oe1)
  edge[arrout] node[lab] {replaced by} (sp);
  
\node[iri,below=2.2\vgap of e1] (sd1) {2014-03-11}
  edge[arrin] node[lab] {start date} (e1);
\node[iri,above=2.2\vgap of e1] (ed1) {2018-03-11}
  edge[arrin] node[lab] {end date} (e1);

\node[iri,below=2.2\vgap of e2] (sd2) {2006-03-11}
  edge[arrin] node[lab] {start date} (e2);
\node[iri,above=2.2\vgap of e2] (ed2) {2010-03-11}
  edge[arrin] node[lab] {end date} (e2);
  
\node[iri,below=\vgap of oe1] (rl) {Ricardo Lagos}
  edge[arrin,bend right=17] node[lab] {replaces} (e2);
\end{tikzpicture}
\caption{Directed edge-labelled graph reifying the statements of Figure~\ref{fig:mb} \label{fig:delg}}
\end{figure}

A number of graph models have been proposed to capture higher-arity relations more concisely, including property graphs~\cite{FrancisGGLLMPRS18} and RDF*~\cite{Hartig17}. However, all of these have limitations that render them incapable of modelling the statements shown in Figure~\ref{fig:mb} without resorting to reification~\cite{HoganRRS19}. Property graphs allow labels and property--value pairs to be associated with both nodes and edges, as shown in Figure~\ref{fig:pg}. Though more concise than reification, labels, properties and values are considered to be simple strings, which are disjoint with nodes; for example, \texttt{"Ricardo Lagos"} is not a node nor a pointer to a node, but a string, which would complicate, for example, querying for the parties of presidents that Michelle Bachelet replaced. On the other hand, RDF* allows an edge to be a node, where Figure~\ref{fig:rdf*} illustrates how it can represent the first statement. However,  we can only represent one of the statements (without reification), as we can only have one distinct node per edge; if we add the qualifiers for both statements, then we would not know which start date pairs with which end date, for example. %Finally, RDF datasets model multiple named graphs, where we could define a graph with a single edge and define qualifiers on that graph's name~\cite{HernandezHK15}; however, named graphs are intended for tracking the source of a graph.


\begin{figure}[t]
\setlength{\vgap}{1.5cm}
\setlength{\hgap}{1cm}
\centering
\begin{tikzpicture}
  %%% node n1 
  \node[nrect] (n1) {
   \alt{
       \uri{given name} & =\,\uri{"Verónica"} } };
  %%% label of n1
  \node[rt] (ln1) at (n1.north) {\uri{human : Michelle Bachelet}};
  
  %%% node n2
  \node[nrect,right=\hgap of n1] (n2) {
   \alt{
      \uri{inception} & =\,\uri{"09 July 1826"} } };
  %%% label of n2
  \node[rt] (ln2) at (n2.north) {\uri{public office: President of Chile}};

  %%% edge e1
  \draw[arrout,pos=0.5,bend left=25] (ln1) to node[rte,yshift=-0.2cm] (le1)
   {\uri{$e_1$ $:$ position held}}
  (ln2);
  %%% atributes e1
  \node[erect,anchor=south,yshift=-0.5ex] at (le1.north) (e1) {
     \alt{ \uri{start date} & =\,\uri{"11 March 2014"}\\[-0.7em]
           \uri{end date} & =\,\uri{"11 March 2018"}\\[-0.7em]
           \uri{replaces} & =\,\uri{"Sebastián Piñera"}\\[-0.7em]
           \uri{replaced by} & =\,\uri{"Sebastián Piñera"} } };
  
  %%% edge e2
  \draw[arrout,pos=0.5,bend right=25] (n1) to node[rte] (le2) {\uri{$e_2$ $:$ position held}} (n2);
  %%% atributes e2  
  \node[erect,anchor=north,yshift=0.5ex] (e2) at (le2.south) {
     \alt{ \uri{start date} & =\,\uri{"11 March 2006"}\\[-0.7em]
           \uri{end date} & =\,\uri{"11 March 2010"}\\[-0.7em]
           \uri{replaces} & =\,\uri{"Ricardo Lagos"}\\[-0.7em]
           \uri{replaced by} & =\,\uri{"Sebastián Piñera"}\\ } };
\end{tikzpicture}
\caption{Property graph for the statements of Figure~\ref{fig:mb}, with some additional data\label{fig:pg}}
\end{figure}

\begin{figure}[tb]
\setlength{\vgap}{0.8cm}
\setlength{\hgap}{1.9cm}
\centering
\begin{tikzpicture}
\node[iri,anchor=center,minimum width=6.3cm,minimum height=0.7cm,dashed] (e1) {};
\node[iri,right=1ex of e1.west,anchor=west] (sp1) {Michelle Bachelet};
\node[iri,right=\hgap of sp1] (ch1) {President of Chile}
  edge[arrin] node[iri,draw=none] {position held} (sp1);
  
\node[iri,below=\vgap of e1] (mb) {Sebastián Piñera}
  edge[arrin,bend right=40] node[lab,xshift=1ex] {replaces} (e1)
  edge[arrin,bend left=40] node[lab,xshift=-1ex] {replaced by} (e1);

\node[iri,left=\hgap of mb] (ttt) {2018-03-11}
  edge[arrin] node[lab] {start date} (e1);

\node[iri,right=\hgap of mb] (ttf) {2014-03-11}
  edge[arrin] node[lab] {end date} (e1);
\end{tikzpicture}
\caption{RDF* graph for the first statement of Figure~\ref{fig:mb} \label{fig:rdf*}}
\end{figure}

\subsection{Domain Graphs}
\label{sec-proposal}

Our data model proposes a simple extension of directed labelled graphs in order to more concisely represent higher-arity relations: each edge of the form \gedge[arrin][1.8cm]{Michelle Bachelet}{position held}{President of Chile} is assigned a unique (possibly internal, autogenerated) identifier that can be used elsewhere in the graph. Figure~\ref{???} illustrates how the statements of Figure~\ref{fig:mb} are represented in our model.

\ah{Giving three alternatives for how to draw the domain graph: Figure~\ref{fig:dg1}, Figure~\ref{fig:dg2}, Figure~\ref{fig:dg3}. We would only use one, whatever is preferred.}
\ra{I like Figure~\ref{fig:dg2}, although it just works for a single level of edge-with-edge.}
\dv{I would still vote for Figure~\ref{fig:dg3}, but putting "edges" into different types of boxes. I can live with the other two as well though.}
\riveros{My vote is for Figure~\ref{fig:dg2}. It is in line of the spirit of Domain graphs. However, it is a bit misleading, because each edge should also have an identifier. I would explain this in the text. }

\begin{figure}[tb]
\setlength{\vgap}{0.8cm}
\setlength{\hgap}{1.9cm}
\centering
\begin{tikzpicture}
\node[iri,anchor=center,minimum width=6.8cm,minimum height=1.3cm,dashed] (e1) {};

\node[anchor=south east,above left=0.1ex of e1.south east,dashed] (e1i) {$e_1$};

\node[iri,right=1ex of e1.west,anchor=west,yshift=1ex] (sp1) {Michelle Bachelet};
\node[iri,right=\hgap of sp1] (ch1) {President of Chile}
  edge[arrin] node[iri,draw=none] {position held} (sp1);
  
\node[iri,anchor=center,minimum width=6.8cm,minimum height=1.3cm,anchor=mid,fill=none,xshift=-4ex,yshift=2ex,dashed] (e2) at (e1) {};

\node[anchor=north west,below right=0.1ex of e2.north west] (e2i) {$e_2$};

\node[iri,below=\vgap of e1] (ttt) {2018-03-11}
  edge[arrin] node[lab] {start date} (e1);
  
\node[iri,left=\hgap of ttt] (mb) {Sebastián Piñera}
  edge[arrin,bend right=20] node[lab,xshift=1ex] {replaces} (e1)
  edge[arrin] node[lab,xshift=-1ex] {replaced by} (e1)
  edge[arrin,bend left=10] node[lab,xshift=-1ex] {replaced by} (e2.190);

\node[iri,right=\hgap of ttt] (ttf) {2014-03-11}
  edge[arrin] node[lab] {end date} (e1);

\node[iri,above=\vgap of e2] (ttt2) {2006-03-11}
  edge[arrin] node[lab] {start date} (e2);
  
\node[iri,left=\hgap of ttt2] (rl) {Richard Lagos}
  edge[arrin] node[lab,xshift=1ex] {replaces} (e2);

\node[iri,right=\hgap of ttt2] (ttf2) {2010-03-11}
  edge[arrin] node[lab] {end date} (e2);

%\node[iri,anchor=center,minimum width=6.6cm,minimum height=0.7cm,below=mb] (e1) {};

%\node[anchor=east,left=0.1ex of e1.east] (e1i) {$e_1$};
\end{tikzpicture}
\caption{Domain graph for Figure~\ref{fig:mb} (v1) \label{fig:dg1}}
\end{figure}

\begin{figure}[tb]
\setlength{\vgap}{0.8cm}
\setlength{\hgap}{1.9cm}
\centering
\begin{tikzpicture}
\node[iri,anchor=center,minimum width=6.6cm,minimum height=0.7cm,dashed] (e1) {};

\node[anchor=south east,above left=0.1ex of e1.south east] (e1i) {$e_1$};

\node[iri,right=1ex of e1.west,anchor=west] (sp1) {Michelle Bachelet};
\node[iri,right=\hgap of sp1] (ch1) {President of Chile}
  edge[arrin] node[iri,draw=none] {position held} (sp1);
  
\node[iri,below=\vgap of e1] (mb) {Sebastián Piñera}
  edge[arrin,bend right=40] node[lab,xshift=1ex] {replaces} (e1)
  edge[arrin,bend left=40] node[lab,xshift=-1ex] {replaced by} (e1);

\node[iri,left=\hgap of mb] (ttt) {2018-03-11}
  edge[arrin] node[lab] {start date} (e1);

\node[iri,right=\hgap of mb] (ttf) {2014-03-11}
  edge[arrin] node[lab] {end date} (e1);
  
\node[iri,anchor=center,below=\vgap of mb,minimum width=6.6cm,minimum height=0.7cm,dashed] (e2) {}
  edge[arrout] node[lab,xshift=-1ex] {replaced by} (mb);

\node[anchor=south east,above left=0.1ex of e2.south east,dashed] (e2i) {$e_2$};

\node[iri,right=1ex of e2.west,anchor=west] (sp2) {Michelle Bachelet};
\node[iri,right=\hgap of sp2] (ch2) {President of Chile}
  edge[arrin] node[iri,draw=none] {position held} (sp2);

\node[iri,below=\vgap of e2] (rl) {Richard Lagos}
  edge[arrin] node[lab] {replaces} (e2);

\node[iri,left=\hgap of rl] (ttt2) {2006-03-11}
  edge[arrin] node[lab] {start date} (e2);

\node[iri,right=\hgap of rl] (ttf2) {2010-03-11}
  edge[arrin] node[lab] {end date} (e2);

%\node[iri,anchor=center,minimum width=6.6cm,minimum height=0.7cm,below=mb] (e1) {};

%\node[anchor=east,left=0.1ex of e1.east] (e1i) {$e_1$};
\end{tikzpicture}
\caption{Domain graph for Figure~\ref{fig:mb} (v2) \label{fig:dg2}}
\end{figure}

\begin{figure}[tb]
\setlength{\vgap}{0.8cm}
\setlength{\hgap}{1.6cm}
\centering
\begin{tikzpicture}
\node[iri,anchor=west,yshift=1ex] (sp1) {Michelle Bachelet};
\node[iri,right=\hgap of sp1] (ch1) {President of Chile}
  edge[arrin,bend left=40] node[fill=white] (e1) {$e_1:$ position held} (sp1)
  edge[arrin,bend right=40] node[fill=white] (e2) {$e_2:$  position held} (sp1);

\node[iri,below=\vgap of e1] (ttt) {2018-03-11}
  edge[arrin] node[lab] {start date} (e1);
  
\node[iri,left=0.5\hgap of sp1] (mb) {Sebastián Piñera}
  edge[arrin,bend right=30] node[lab,xshift=1ex] {replaces} (e1)
  edge[arrin,bend right=10] node[lab,xshift=-1ex] {replaced by} (e1)
  edge[arrin,bend left=20] node[lab,xshift=-1ex] {replaced by} (e2);

\node[iri,right=0.5\hgap of ttt] (ttf) {2014-03-11}
  edge[arrin] node[lab,xshift=1ex] {end date} (e1);

\node[iri,above=\vgap of e2] (ttt2) {2006-03-11}
  edge[arrin] node[lab] {start date} (e2);
  
\node[iri,left=0.5\hgap of ttt2] (rl) {Richard Lagos}
  edge[arrin] node[lab] {replaces} (e2);

\node[iri,right=0.5\hgap of ttt2] (ttf2) {2010-03-11}
  edge[arrin] node[lab,xshift=1ex] {end date} (e2);

%\node[iri,anchor=center,minimum width=6.6cm,minimum height=0.7cm,below=mb] (e1) {};

%\node[anchor=east,left=0.1ex of e1.east] (e1i) {$e_1$};
\end{tikzpicture}
\caption{Domain graph for Figure~\ref{fig:mb} (v3) \label{fig:dg3}}
\end{figure}

Formally, assume a countably infinite set $\objs$ of objects. We can define a domain graph as follows:
\riveros`{I would aim the presentation to VLDB people. Saying ``countably infinite'' has no practical implications for the model and it only scares a potential VLDB reviewer.}

\begin{definition}
A \emph{domain graph} $G = (O,\gamma)$ consists of a finite set of objects $O\subseteq \objs$ and a partial mapping $\gamma : O \rightarrow O \times O \times O$.
\end{definition}

\ra{Is an object an identifier, a label, a value, the three above?}
\dv{This is explained below, but I agree that mentioning it as qualifiers is a bit confusing.}

Alternatively we can define our model as a relation:
\[\textsc{DomainGraph}(\textsf{source},\textsf{type},\textsf{target},\underline{\textsf{eid}}) \]
where \underline{\textsf{eid}} is a primary key of the relation. 
\riveros{I would show here an example of how the relation of the running example would look. This will help to be more concrete about the model. }

In essence, one could argue that everything in domain graphs is a node, since it can be later referenced again in the mapping $\gamma$. This way domain graphs avoid the aforementioned limitations of other models. When compared with property graphs, the values of the qualifiers are nodes, not strings, which allows us to directly query for other edges involving that node. Compared with RDF*, we can have multiple nodes (with different identifiers) for the same edge. Compared with both, we can ``nest'' qualifiers without issue given that the edges encoding qualifiers themselves have identifiers, which we can use as nodes. We can also represent graphs in other models as domain graphs. Representing RDF* is direct: we simply assign identifiers to edges. In the case of property graphs, node labels can be modelled with an edge like \gedge[arrin]{Michelle Bachelet}{label}{human}, while property--value pairs on nodes or edges can be modelled as edges emanating from those nodes or edges.

\ah{We could define property domain graphs here in more detail, if preferred.}

Of course, features of the property graph data model such as node labels, or properties with their values, offer practical advantages when filtering classes of nodes and/or edges, as well as allowing to specify non trivial path constraints that are not captured purely by edge \textsf{types}. For this reason, and to ensure backwards compatibility with property graphs, in MillenniumDB we actually support an extended version of domain graphs, called property domain graphs.

\begin{definition}
%Let $L$ be a set of labels, $K$ a set of keys/attributes, and $V$ a set of atomic values (e.g. ints, strings, floats, dates, etc.).
 A \emph{property-\data} is defined as a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
    \item $(O,\gamma)$ is a \data;
    \item $\lab : O \mapsto 2^\labels$ is the labelling function assigning a finite set of labels to each object; and
    \item $\prop : O \times \keys \mapsto \values$ is a partial function assigning a value of a certain key (property) of some object, to its value.
\end{itemize}
\end{definition}
\riveros{I would specify $\labels$, $\keys$, and $\values$ in the definition of the model.}

In brief, \data capture the graph structure of our model, while property-\data additionally allow to assign labels and key value pairs to objects, as ordinary property graphs do.
A relational representation of property-\data would then contain the following two relations, in addition to the \textsc{DomainGraph} specified above:
\[\textsc{Labels}(\textsf{object},\textsf{label})\]
\[\textsc{Properties}(\underline{\textsf{object},\textsf{key}},\textsf{value})\]
where \underline{\textsf{object, key}} is a primary key of the second relation, with the first relation allowing multiple labels per object. 

To sum, up the full data model supported by MillenniumDB allows the user to treat their graph as a:
\begin{itemize}
\item Standard property graph (by ignoring quantifiers and nested structures).
\item RDF graph (the \data model already accomplishes this by ignoring the edge id).
\item Wikidata \cite{VrandecicK14} knowledge graph which uses qualifiers that can again be nodes/objects.
\item Property graph with nested qualifiers (i.e. the full data model).
\end{itemize} 

We note that an exploration of the expressive power of this data model lies outside of the scope of this paper, so we omit it here. 
\riveros{Maybe I would add in the appendix ``simple'' translations of the main models in the literature to property-domain graphs. This is important for convincing the reader that the model is natural.}
As a side note in this direction, nested qualifiers actually allow the \data model to express features that are outside of the scope of hypergraphs.

==> sections/data.tex <==
%!TEX root = ../main.tex

In this section, we first introduce some of the most popular data models that have been used for graph databases. We then discuss the model that MillenniumDB uses -- called \textit{domain graphs} -- that generalises these other models. In order to exemplify these models, we will take examples from Wikidata~\cite{VrandecicK14}: a prominent, multilingual, open and collaboratively-edited knowledge graph.

\subsection{Popular Graph Data Models}

A number of graph-based data models have become popular in recent years~\cite{AnglesABHRV17}. Perhaps the simplest such model is that of \textit{directed labelled graphs}, that is a set of nodes and edges such that every edge relates a pair of nodes. An edge is graphically represented as \gedge[arrin][0.6cm]{$a$}{$b$}{$c$}, where $a$ is called the source node, $b$ the edge label, and $c$ the target node. A real example of edge might be \gedge[arrin][2cm]{Michelle Bachelet}{position held}{President of Chile}. Hence, nodes are used to represent entities and edges represent binary relations.  
%A popular concrete model based on \textit{directed edge-labelled graphs} is the RDF model~\cite{CyganiakWL14}. 

While directed labelled graphs work straightforwardly for representing binary relations, things become more complicated if we wish to consider higher arity relations, such as to indicate \textit{when} Michelle Bachelet held the position of President of Chile. Figure~\ref{fig:mb} presents a statement group from the Wikidata knowledge graph~\cite{VrandecicK14} where labels are presented in English for readability. This example contains two statements relating to two different presidencies of \texttt{Michelle Bachelet}. Each statement is associated with its own \textit{qualifiers}, including \texttt{start date} and \texttt{end date}, whom she was replaced by, and whom she replaced. Statements may also be associated with ranks, references, and so forth. Complex statements like this can be cumbersome to be represent as a directed labelled graph, requiring some form of \textit{reification} to decompose $n$-ary relations into binary relations~\cite{HernandezHK15}. For example, Figure~\ref{fig:delg} shows a graph where $e_1$ and $e_2$ are nodes representing $n$-ary relationships. The reification is given by the use of the edges labelled as \texttt{source node}, \texttt{edge} and \texttt{target node}. 

%\newcommand{\wid}[1]{{\color{gray}~[#1]}} % format Wikidata IDs

\begin{figure}[tb]
\centering
{\sf
\begin{tabular}{l}
\large\textbf{Michelle Bachelet\wid{Q320}}\\[1ex]
\large\qquad position held\wid{P39} \quad President of Chile\wid{Q466956}\\
\qquad \qquad 
{\begin{tabular}{l@{\qquad~~}l}
start date \wid{P580} & 2014-03-11\\
end date \wid{P582} 	& 2018-03-11\\
replaces\wid{P155}	& Sebastián Piñera\wid{Q306}\\
replaced by\wid{P156} & Sebastián Piñera\wid{Q306}\\
\end{tabular}}\\
\\[-1ex]
\large\qquad position held\wid{P39} \quad President of Chile\wid{Q466956}\\
\qquad \qquad {\begin{tabular}{l@{\qquad~~}l}
start date \wid{P580} & 2006-03-11\\
end date \wid{P582} & 2010-03-11\\
replaces\wid{P155} & Ricardo Lagos\wid{Q331}\\
replaced by\wid{P156} & Sebastián Piñera\wid{Q306}\\
\end{tabular}}
\end{tabular}
}
\caption{Wikidata statement group for Michelle Bachelet \label{fig:mb}}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=8.5cm]{./images/digraph.png}
\caption{Directed edge-labelled graph reifying the statements of Figure~\ref{fig:mb} \label{fig:delg}}
\end{figure}


%\begin{figure}[t]
%\setlength{\vgap}{0.7cm}
%\setlength{\hgap}{1.4cm}
%\centering
%\begin{tikzpicture}
%\node[iri] (e1) {$e_1$};
%\node[iri,right=\hgap of e1] (pe1) {P39}
%  edge[arrin] node[lab] {pred} (e1);
%\node[iri,above=\vgap of pe1] (se1) {Q320}
%  edge[arrin,bend right=10] node[lab] {subj} (e1);
%\node[iri,below=\vgap of pe1] (oe1) {Q466956}
%  edge[arrin,bend left=10] node[lab] {obj} (e1);
%\node[iri,above=\vgap of se1] (sp) {Q306}
%  edge[arrin,bend right=13] node[lab] {P155} (e1)
%  edge[arrin,bend right=45] node[lab] {P156} (e1);
%\node[iri,left=1.6\hgap of se1] (sd1) {2014-03-11}
%  edge[arrin] node[lab] {P580} (e1);
%\node[iri] (ed1) at (sd1|-oe1) {2018-03-11}
%. edge[arrin] node[lab] {P582} (e1);
%\node[iri,right=\hgap of pe1] (e2) {$e_2$}
%  edge[arrout] node[lab] {pred} (pe1)
%  edge[arrout,bend right=10] node[lab] {subj} (se1)
%  edge[arrout,bend left=10] node[lab] {obj} (oe1)
%  edge[arrout,bend right=45] node[lab] {P156} (sp);
%\node[iri,right=1.6\hgap of se1] (sd2) {2006-03-11}
%  edge[arrin] node[lab] {P580} (e2);
%\node[iri] (ed2) at (sd2|-oe1) {2018-03-11}
%  edge[arrin] node[lab] {P582} (e2);
%\node[iri,below=\vgap of e2] (rl) {Q331}
%  edge[arrin] node[lab] {P155} (e2);
%\end{tikzpicture}
%\caption{Directed edge-labelled graph reifying the statements of Figure~\ref{fig:mb} \label{fig:delg}}
%\end{figure}

Using reification may make the graph model less intuitive, and may be verbose in terms of using several edges to represent one relation. An alternative is to use a model able to represent higher-arity relationships. Among the most popular alternatives are property graphs~\cite{FrancisGGLLMPRS18}, RDF datasets~\cite{CyganiakWL14}, and RDF*~\cite{Hartig17}. 
%Each of these models has supporting query languages~\cite{FrancisGGLLMPRS18,HarrisS13,Hartig17}.

In property graphs, both nodes and edges can be associated with an id, a label, and one or more key--value pairs called properties. Figure~\ref{fig:pg1} shows a property graph for the statements of the running example.
Note that the two presidencies of \texttt{Michell Bachellet} are represented by using two different edges, and the specific qualifiers are represented as properties of such edges. 
Although we are have solved the problem found by using a directed labelled graph (i.e. the use of reification for representing n-ary relations), we can observe that we are not able to associate more information to the properties of nodes and edges (e.g. \texttt{Sebastián Piñera} is a simple value instead of node that can be described). The later implies that the property graph model does not support relationships with multiple levels of descriptions or qualifiers. 

%However, there are some limitations in terms of how property graphs are implemented and how they are queried in systems such as Cypher/Neo4j~\cite{FrancisGGLLMPRS18}. Properties cannot take multiple values (e.g., for multilingual labels), properties are not intended to take edge IDs as values, indexes are not supported for properties on edges, etc. 
%Aside from the specific implementation of Neo4j, the property graph model is quite verbose, and it is not directly clear how it should be physically represented and indexed.

\begin{figure}[t]
\centering
\includegraphics[width=8cm]{./images/pg1.png}
\caption{Property graph for the statements of Figure~\ref{fig:mb}.\label{fig:pg1}}
\end{figure}

%\begin{figure}[t]
%\setlength{\vgap}{1.5cm}
%\setlength{\hgap}{1cm}
%\centering
%\begin{tikzpicture}
  %%%% node n1 
%  \node[nrect] (n1) {
%   \alt{
%       \uri{label} & =\,\uri{Michelle Bachelet@en} } };
   %%%% label of n1
%  \node[rt] (ln1) at (n1.north) {\uri{Q5 : Q320}};
 %%%% node n2
%  \node[nrect,right=\hgap of n1] (n2) {
%   \alt{
%      \uri{label} & =\,\uri{President of Chile@en} } };
  %%%% label of n2
%  \node[rt] (ln2) at (n2.north) {\uri{Q294414 : Q466956}};
  %%%% edge e1
%  \draw[arrout,pos=0.5,bend left=50] (ln1) to 
%   node[erect] (e1) {
%   \alt{ \uri{P580} & =\,\uri{"11 March 2014"}\\
%         \uri{P582} & =\,\uri{"11 March 2018"}\\
%         \uri{P155} & =\,\uri{Q306}\\
%         \uri{P156} & =\,\uri{Q306}\\ } }
%  (ln2);
   %%%% label of e1
%  \node[rte] (le1) at (e1.north) {\uri{P39 $:$ $e_2$}};
   %%%% edge e1
%  \draw[arrout,pos=0.5,bend right=65] (n1) to 
%   node[erect] (e1) {
%   \alt{ \uri{P580} & =\,\uri{"11 March 2006"}\\
%         \uri{P582} & =\,\uri{"11 March 2010"}\\
%         \uri{P155} & =\,\uri{Q331}\\
%         \uri{P156} & =\,\uri{Q306}\\ } }
%  (n2);  
  %%%% label of e1
%  \node[rte] (le1) at (e1.north) {\uri{P39 $:$ $e_1$}};
%\end{tikzpicture}
%\caption{Property graph for the statements of Figure~\ref{fig:mb}; additionally, \urit{Q294414} refers to \textsf{public office} (a type)\label{fig:pg}}
%\end{figure}

Regarding RDF*~\cite{Hartig17}, the idea is to allow statements about statements, i.e. we can add edges to an edge. We illustrate this idea in Figure~\ref{fig:rdf-star}, where the statement \gedge[arrin][2cm]{Michelle Bachelet}{position held}{President of Chile} has been associated with qualifiers and other meta-data.  While this approach might appear promising at first glance, the two statements of Figure~\ref{fig:mb} cannot be distinguished as the model does not support multiple instances of the same statement; this would then conflate the qualifiers for the two presidencies.

\begin{figure}[t]
\centering
\includegraphics[width=8cm]{./images/rdf-star.png}
\caption{RDF* representation of the first statement of Figure~\ref{fig:mb} \label{fig:rdf-star}}
\end{figure}

%\begin{figure}[tb]
%\setlength{\vgap}{0.9cm}
%\setlength{\hgap}{2cm}
%\centering
%\begin{tikzpicture}
%\node[iri,anchor=center,minimum width=4.4cm,minimum height=0.7cm] (e1) {};
%\node[iri,right=1ex of e1.west,anchor=west] (sp1) {Q320};
%\node[iri,right=\hgap of sp1] (ch1) {Q466956}
%  edge[arrin] node[iri,draw=none] {P39} (sp1);
%\node[iri,right=\hgap of e1] (ttt) {2018-03-11}
%  edge[arrin] node[lab] {P580} (e1);
%\node[iri,above=0.5\vgap of ttt] (ttf) {2014-03-11}
%  edge[arrin] node[lab] {P582} (e1);
%\node[iri,below=0.5\vgap of ttt] (mb) {Q306}
%  edge[arrin,bend right=6] node[lab] {P155} (e1)
%  edge[arrin,bend left=6] node[lab] {P156} (e1);
%\end{tikzpicture}
%\caption{RDF* representation of the first statement of Figure~\ref{fig:mb} \label{fig:rdf*}}
%\end{figure}



\ma{If we want to distinguish the two statements of Figure~\ref{fig:mb}, couldn't we use two identifiers for the triple? In RDF* this could be written as follows:

\urit{t1} \urit{represents} <<\urit{Q320} \urit{P39} \urit{Q466956}>>

\urit{t2} \urit{represents} <<\urit{Q320} \urit{P39} \urit{Q466956}>>

And then we can use either \urit{t1} or \urit{t2} depending on the triple we are making reference to.
}

\ah{Yep, but then you are reifying the triple, and reification is precisely what RDF* is trying to avoid. :) Here, \urit{t1} and \urit{t2} represent the statements, which are basically the nodes $e_1$ and $e_2$ of Figure~\ref{fig:delg}. Maybe this could be clarified ...}

% \ma{In Figure \ref{fig:rdf*}, should \urit{Q466956} be replaced by \urit{Q11696}? What does \urit{Q466956} represent?} % ah: Fixed

Finally we have RDF datasets~\cite{CyganiakWL14}, supported in SPARQL as named graphs~\cite{HarrisS13}, where multiple graphs can be defined and managed as a single instance. In this setting we can assign each statement to its own named graph, and then use the graph's name to define meta-data on the statement~\cite{HernandezHK15}. However, this approach has some practical limitations. Foremost of these, the model considers multiple distinct graphs rather than one graph; as a result, for example, path queries in SPARQL cannot be applied over multiple graphs at once, requiring either a default graph to be defined as the union of all graphs, or requiring the graphs on which the path should be applied to be explicitly named in the query.

%Aside from these issues, there are also continued debates about how to handle complex objects in graphs, such as lists, values with precision, dates with calendars, multidimensional values such as geographic points, measures with units, multilingual strings, etc. Wikidata~\cite{VK14:Wikidata} contains a range of these complex objects.
%\noindent

These models are the most popular for graph databases in practice. Although they have different strengths and weaknesses, they all follow a graph abstraction and are thus interoperable, where one can convert data from one model to the other with relative ease (possibly using reification if moving from higher to lower arity). 
%We would like to support all such models in MillenniumDB.

%======
\subsection{Property-Domain Graphs}
\label{sec-proposal}
In this section we introduce the notion of property-domain graph, which is the data model used in MillenniumDB.
The property-domain graph model extends the property graph model by allowing edges between edges, without any kind of restriction. This extension allows a multi-dimensional representation of relationships. 

Assume an infinite set $\labels$ of labels, and a set $\values$ of atomic values  (e.g. integers, strings, floats, dates, etc.). 
\begin{definition}[Property-domain graph] 
 A property-domain graph is a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
\item $O$ is a finite set of object identifiers;
\item $\gamma : O \to O \times O \times O$ is a partial function that associates objects with a tuple of three objects; 
\item $\lab : O \to \labels$ is a partial function that associates objects with labels; and
\item $\prop : O \times \labels \to \values$ is a partial function that associates objects with labels and values (i.e. properties).
\end{itemize}
\end{definition}

 \begin{figure}[t]
\centering
\includegraphics[width=8.5cm]{./images/dgraph.png}
\caption{Property-domain graph for the statements of Figure~\ref{fig:mb}. \label{fig:dgraph}}
\end{figure}

The set $O$ is called the \textit{domain}, referring to both the universe of objects, and the domain of the function $\gamma$.
Each object in $O$ have a single identifier, zero or one label (defined by function $\lab$), and zero or many properties (defined by function $\prop$). In terms of data modeling, an object can represent an entity, a relationship (when it is in the domain of $\gamma$), or both.

An example of property-domain graph is presented in Figure \ref{fig:dgraph}.
We use different shapes to represent the componentes of an object: the object identifier and the label is inside a rounded square (e.g. $o_1:$ \texttt{Person}); the properties are inside a square (e.g. \texttt{Name = ``Michelle bachelet''}), and the 3-tuple associate to an object is inside a rounded dotted square (e.g. \gedge[arrin][1cm]{$o_1$}{$o_4$}{$o_5$}).

The objects are organized in groups called \emph{representation levels}.
Level 1 contains objects representing simple entities (e.g. $o_4:$) or complex entities (e.g. $o_1$).
Level 2 contains objects representing relations among the entities of level 1.
Level 3 contains objects from the lower leves, and so on.
 
Note that the property-domain graph is compatible with other graph models.
In fact, we just need a two-level property-domain graph to represent directed labeled graphs, RDF* graphs and named graphs.

%An important property of \datas is that they can be directly represented in the relational model and indexed straightforwardly. A \data can viewed as a single quaternary relation $Q(S,P,O,\underline{E})$, with primary key $E$, such that $\gamma(E)=(S,P,O)$. We will speak in more detail about indexing later in Section~\ref{sec:storage}.







%======
\subsection{Domain Graphs (OLD, TO BE REMOVED)}
\label{sec-proposal}

We now define the graph data model used in MillenniumDB in order to generalise the aforementioned models used in practice. Assume a countably infinite set $\objs$ of objects.

\begin{definition}
A \emph{domain graph} $G = (O,\gamma)$ consists of a finite set of objects $O\subseteq \objs$ and a partial mapping $\gamma : O \rightarrow O \times O \times O$.
\end{definition}

The set $O$ is called the \textit{domain}, referring to both the universe of objects, and the domain of the function $\gamma$. Objects in $O$ may be either primitive or complex objects. Primitive objects include strings, IRIs, integers, existential variables, non-existential values, etc. Complex objects may include values with datatypes, units, precision, or languages; sets, bags, or ordered tuples/lists of values; items with nested ids, labels, property--value attributes, etc. Complex objects can often be replaced by primitive nodes described in the graph itself (as a classical example, RDF lists provide a mechanism for representing ordered terminated lists within an RDF graph without need for a dedicated list object~\cite{CyganiakWL14}). However, such representations might end up being verbose and inefficient to cope with. On the other hand, each new type of complex object requires higher level tools and languages to have dedicated logic and features to be able to correctly interpret and work with that object. We abstract away such details, assuming that graphs representing such objects can be lifted (to complex objects) and lowered (to a sub-graph of more primitive objects) as needs be. The domain of $\gamma$ can be handled internally by the database or externally by the user/dataset; the image of $\gamma$ (a graph) can also be queried independently of its domain.

The \data itself can be conceptualised in a number of ways. We can think of it as a directed edge-labelled graph (e.g., an RDF graph), where each edge has a unique identifier that makes it an object. Or we may consider it as akin to a directed labelled multigraph (sometimes known as a \emph{labelled quiver}).

An example of a \data representing the two statements of Figure~\ref{fig:mb} is given in Figure~\ref{fig:doma}. Here an object that is also a connection id (aka.\ an edge id) is denoted with lower case $e$. For example $\gamma(e_1) = (\texttt{Q320},\texttt{P39},\texttt{Q466956})$. The object $e_1$ then participates in two other connections $e_3$, and $e_4$. These can again be connected to other objects. Intuitively, in  $\gamma(e_1) = (\texttt{Q320},\texttt{P39},\texttt{Q466956})$, $e_1$ represents a connection between $\texttt{Q320}$ and $\texttt{Q466956}$, and $\texttt{P39}$ is a descriptor, or type/label of this connection. The descriptor itself can then be part of a connection, as is the case with, for instance, $\texttt{P39}$ in Figure~\ref{fig:mb}.


%\begin{figure*}[tb]
%\setlength{\vgap}{1.4cm}
%\setlength{\hgap}{4cm}
%\centering
%\begin{tikzpicture}
%
%\node[iri,right=1ex of e1.west,anchor=west] (sp1) {Q320};
%
%\node[iri,right=\hgap of sp1] (ch1) {Q466956}
%  edge[arrin,bend right=10] node[var] (e1) {$e_1$ : P39} (sp1)
%  edge[arrin,bend left=10] node[var] (e2) {$e_2$ : P39} (sp1);
%
%\node[iri,above=\vgap of e1,xshift=2cm] (tt1) {\dtt{2018-03-11}{xsd:date}}
%  edge[arrin] node[var] (e3) {$e_4$ : P582} (e1);
%  
%\node[iri,above=\vgap of e1,xshift=-2cm] (tt2) {\dtt{2014-03-11}{xsd:date}}
%  edge[arrin] node[var] (e4) {$e_3$ : P580} (e1);
%  
%\node[iri,right=\hgap of ch1] (sp) {Q306}
%  edge[arrin,bend right=10] node[var] (e5) {$e_6$ : P155} (e1)
%  edge[arrin,bend right=24] node[var] (e6) {$e_5$ : P156} (e1)
%  edge[arrin,bend left=10] node[var] (e7) {$e_7$ : P155} (e2);
%
%\node[iri,below=\vgap of sp] (rl) {Q331}
%  edge[arrin,bend left=8] node[var] (e8) {$e_8$ : P156} (e2);
%
%\node[iri,below=\vgap of e2,xshift=2cm] (tt1) {\dtt{2010-03-11}{xsd:date}}
%  edge[arrin] node[var] (e9) {$e_9$ : P582} (e2);
%  
%\node[iri,below=\vgap of e2,xshift=-2cm] (tt2) {\dtt{2006-03-11}{xsd:date}}
%  edge[arrin] node[var] (e10) {$e_{10}$ : P580} (e2); 
%\end{tikzpicture}
%
%\caption{Domain graph representation of the two statements of Figure~\ref{fig:mb} \label{fig:doma}}
%\end{figure*}

%Per Figure~\ref{fig:mb}, we claim that \data allows for modelling Wikidata almost immediately; in fact, the \data model is even more expressive as it allows to have quantifiers on quantifiers on quantifiers, etc. 

An important property of \datas is that they can be directly represented in the relational model and indexed straightforwardly. A \data can viewed as a single quaternary relation $Q(S,P,O,\underline{E})$, with primary key $E$, such that $\gamma(E)=(S,P,O)$. We will speak in more detail about indexing later in Section~\ref{sec:storage}.

\Datas also have the advantage of being compatible with other proposed models. For instance, they can model RDF graphs immediately: the range of $\gamma$ is a directed-edge labelled graph. 

Similarly, RDF* graphs are also representable as a \data by either allowing RDF triples as complex objects, or by lowering, e.g., $((s,p,o),p',o')$ to $\gamma(e_1) = (s,p,o)$, $\gamma(e_2) = (e_1,p',o')$.

Likewise although RDF datasets are more general than \data, being representable as a relation $D(S,P,O,G)$ without $G$ being a primary key (here assuming a fixed IRI for the default graph), we can represent $(s,p,o,g)$ as $\gamma(e_1) = (s,p,o)$, $\gamma(e_2) = (e_1,\texttt{graph},g)$.

Additionally, if one allows complex objects in $O$ with labels and properties, they can also simulate property graphs in a direct way. More precisely, assuming a set $\labels$ of labels, a set $\keys$ of keys/attributes, and a set $\values$ of atomic values  (e.g. ints, strings, floats, dates, etc.), we define property-\datas as follows:

\begin{definition}[Property-\data] 
%Let $L$ be a set of labels, $K$ a set of keys/attributes, and $V$ a set of atomic values (e.g. ints, strings, floats, dates, etc.).
 A property-\data is a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
    \item $(O,\gamma)$ is a \data;
    \item $\lab : O \mapsto 2^\labels$ is the labelling function assigning a finite set of labels to each object; and
    \item $\prop : O \times \keys \mapsto \values$ is a partial function.
\end{itemize}
\end{definition}

Each (multi-valued) property graph $G = (V,E,\rho,\lambda,\sigma)$, as defined in \cite{AnglesABHRV17}, is immediately modelled as a property-\data $G' = (O,\gamma,\lab,\prop)$, where $O = V\cup E$,  $\gamma(o) = (o_1,\varepsilon,o_2)$ whenever $\rho(o) = (o_1,o_2)$, $\lab(o) = \lambda(o)$, and $\prop(o,k)=\sigma(o,k)$. The intermediate node $\varepsilon$ is not used and can be removed for indexing; alternatively, if edges are restricted to have precisely one label (per Cypher/Neo4j~\cite{FrancisGGLLMPRS18}), then we can define $\varepsilon = \lab(o)$ and use $\lab$ for node labels only (now with $O = V\cup E \cup L$). To query on label and property data, auxiliary indexes would be required for $\lab$ and $\prop$. As an alternative to adding auxiliary indexes, the property-\data can be lowered to remove $\texttt{lab}$ and $\texttt{prop}$ on complex objects, representing $\lab(o) = \{ l_1,\ldots,l_m \}$ as $\gamma(e_{l1}) = (o,\texttt{lab},l_1), \ldots, \gamma(e_{lm}) = (o,\texttt{lab},l_m)$, and representing $\prop(o,k) = \{ v_1,\ldots,v_n \}$ as $\gamma(e_{p1}) = (o,k,v_1), \ldots, \gamma(e_{ln}) = (o,k,v_n)$ (now with $O = V\cup E \cup L \cup K \cup V$).


%======
\subsection{Analysis of data models}
\label{sec-models}

\subsubsection{Data model 1}.

Assume an infinite set $\objs$ of object identifiers, an infinite set $\labels$ of labels, and a set $\values$ of atomic values  (e.g. integers, strings, floats, dates, etc.). 
A property-domain graph is a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
\item $O \subset \objs$ is a finite set of object identifiers;
\item $\gamma : O \to O \times O \times O$ is a partial function that associates objects with a tuple of three objects; 
\item $\lab : O \to \labels$ is a partial function that associates objects with labels; and
\item $\prop : O \times \labels \to \values$ is a partial function that associates objects with labels and values (i.e. properties).
\end{itemize}

\begin{itemize}
\item It is a merge of the hypegraph data model (where edges can connect more than two nodes) and the hypernode data model (where a node can be a graph).
\item The function $\gamma$ is not compatible with the traditional notion of  (property) graph where an edge connects a pair of nodes.
\item The transversal use of labels for objects and properties simplify its definition and understanding.
\end{itemize}


\subsubsection{Data model 2}.

\newcommand{\type}{\operatorname{type}}

Assume an infinite set $\objs$ of object identifiers, an infinite set $\labels$ of labels,  a set $\keys$ of keys/attributes, and a set $\values$ of atomic values  (e.g. integers, strings, floats, dates, etc.). 
A property-domain graph is a tuple $G=(O,\gamma,\type,\prop)$, where:
\begin{itemize}
\item $O \subset \objs$ is a finite set of object identifiers;
\item $\gamma : O \to O \times O$ is a partial function; 
\item $\type$ is a subset of $O \times O$; 
\item $\prop : O \times \keys \to \values$ is a partial function.
\end{itemize}

Notes:
\begin{itemize}
\item The difference with Data Model 1 is the definition of the $\gamma$ function.
\item It is compatible with traditional (property) graphs as an edge is a pair of nodes.
\item Function $\type$ is a little confusing. It implies that any object can be a node, an edge, or a type. 
\item The representation power could be higher than Data Model 1.  
\end{itemize}

\subsubsection{Data model 3}.

Assume an infinite set $\objs$ of object identifiers, an infinite set $\labels$ of labels, and a set $\values$ of atomic values  (e.g. integers, strings, floats, dates, etc.). 
A property-domain graph is a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
\item $O \subset \objs$ is a finite set of object identifiers;
\item $\gamma : O \to O \times O$ is a partial function; 
\item $\lab : O \to \labels$ is a partial function that associates objects with labels; and
\item $\prop : O \times \labels \to \values$ is a partial function that associates objects with labels and values (i.e. properties).
\end{itemize}

Notes:
\begin{itemize}
\item The difference with Data Model 1 is the definition of the $\gamma$ function.
\item It is compatible with traditional (property) graphs as an edge is a pair of nodes.
\item The transversal use of labels for objects and properties simplify its definition and understanding.
\item It seems to have the same representation power than Data Model 1.  
\end{itemize}


%======
\subsection{Query language for Data Model 3}
\label{sec-op1}

\smallskip
\noindent
\textbf{Data model}

Assume an infinite set $\objs$ of object identifiers, an infinite set $\labels$ of labels, and a set $\values$ of atomic values  (e.g. integers, strings, floats, dates, etc.). 
 A property-domain graph is a tuple $G=(O,\gamma,\lab,\prop)$, where:
\begin{itemize}
\item $O \subset \objs$ is a finite set of object identifiers;
\item $\gamma : O \to O \times O$ is a partial function (used to define edges); 
\item $\lab : O \to \labels$ is a partial function that associates objects with labels; and
\item $\prop : O \times \labels \to \values$ is a partial function that associates objects with labels and values (i.e. properties).
\end{itemize}

The set $O$ is called the \textit{domain}, referring to both the universe of objects, and the domain of the function $\gamma$.
Each object in $O$ have a single identifier, zero or one label (defined by function $\lab$), and zero or many properties (defined by function $\prop$). In terms of data modeling, an object can represent an entity, a relationship (when it is in the domain of $\gamma$), or both.

\smallskip
\noindent
\textbf{Query language syntax}.

Assume a countably infinite set $\vars$ of variables disjoint with the set of objects $\objs$.

An \textit{path expression} \texttt{p} is defined recursively as as follows:
\begin{itemize}
\item if $a \in labels$ then $a$ is a simple path expression, and $\hat{ }a$ is an inverse path expression;
\item if $p_1$ and $p_2$ are path expressions then
 \begin{itemize}
  \item $p_1 \slash p_2$ is a sequence path expression;
  \item $p_1 + p_2$ is an alternative path expression;
  \item $p_1^*$ is a zero-or-more path expression;
  \item $e?$ is a zero-or-one path expression; 
 \end{itemize}
\end{itemize}

Let $t_1, t_2, t_3 \in \objs \cup \vars$ and $p$ be a path expression.
A \emph{graph pattern} is defined recursively as follows:
A tuple $(t_1,t_2,t_3)$ is a graph pattern called \emph{simple pattern};
A tuple $(t_1, p, t_2)$ is a graph pattern called \emph{path pattern}; 
If $P_1$ and $P_2$ are graph patterns then $(P_1 \AAND P_2)$ and $(P_1 \OPT P_2)$ are complex graph patterns.

A \emph{selection condition} is defined recursively as follows:
(a) If $?X,?Y \in \vars$, $p,q \in \labels$ and $a \in \values$ then $({?X} = {?Y})$, ${label(?X)} = {p}$, ${label(?X)} = {label(?Y)}$, ${?X.p} = {?Y.q}$, ${?X.p} = {a}$ are atomic selection conditions;
(b) If $C_1, C_2$ are selection conditions then $(C_1 \land C_2)$, $(C_1 \lor C_2)$ and $(\neg C_1)$ are complex selection conditions.

Let $?X \in \vars$, $p \in \labels$ and $q \in \labels$.
A \emph{projection function} is any of the following expressions: $?X \AS p$, $o.p \AS  q$, $label(?X) \AS q$.  
A \emph{projection clause} is a set of projection functions. 

A \emph{query} is a tuple $(S,P,C)$ where $S$ is a projection function, $P$ is a graph pattern, and $C$ is a selection condition. 
 
\smallskip 
\noindent
\textbf{Query language semantics}


A \textit{solution mapping} (or simply \textit{mapping}) is a partial function $\map: \vars \rightarrow \objs$. 
The \emph{domain} of a mapping $\map$, denoted $\Dom{\map}$, is the set of variables on which $\map$ is defined.
Given $?X \in \vars$ and $o \in \objs$, we use $\mu(?X) = o$ to denote that $\mu$ maps variable $?X$ to object $o$.  
Additionally, we will assume that $\mu(o)=o$, for all $o\in \objs$. 
%Given a finite set of variables $W$, the restriction of a mapping $\mu$ to $W$, denoted $\mu_{|W}$, is a mapping $\mu'$ which satisfies that $\dom(\mu') = W \cap \dom(\mu)$ and $\mu'(?X) = \mu(?X)$ when $?X \in \dom(\mu')$.

Two mappings $\mu_1, \mu_2$ are \emph{compatible}, denoted $\mu_1 \sim \mu_2$, when for all $?X \in \dom(\mu_1) \cap \dom(\mu_2)$ it satisfies that $\mu_1(?X)=\mu_2(?X)$. 
Note that two mappings with disjoint domains are always compatible.
The union of compatible mappings, denoted $\mu_1 \cup \mu_2$, is also a mapping. 

Let $\Omega_1$ and $\Omega_2$ be sets of mappings.
The operations of join, union, difference and left outer-join between $\Omega_1$ and $\Omega_2$ are defined as follows:
\begin{verse}
$\Omega_1 \Join \Omega_2  = \{ \mu_1 \cup \mu_2 \mid \mu_1 \in \Omega_1 ~\land~ \mu_2 \in \Omega_2 ~\land~ \mu_1 \sim \mu_2 \}$

$\Omega_1 \cup \Omega_2  = \{ \mu \mid \mu_1 \in \Omega_1 ~\lor~ \mu_2 \in \Omega_2 \}$

$\Omega_1 \setminus \Omega_2  = \{ \mu _1 \in \Omega_1 \mid \forall \mu_2 \in \Omega_2, \text{ is false that } \mu_1 \sim \mu_2  \}$

$\Omega_1 \LOJ \Omega_2  = (\Omega_1 \Join \Omega_2) \cup (\Omega_1 \setminus \Omega_2) \}$
\end{verse}

The semantics of selection conditions is defined as follows. 
Given a selection condition $C$, a mapping $\mu$, and a graph $G=(O,\gamma,\lab,\prop)$, we say that $\mu$ satisfies $C$ under $G$, denoted by $\mu \models_G C$, if.  
\begin{itemize}
\item 
$C$ is ${?X} = {?Y}$, $?X \in \dom(\mu)$, $?Y \in \dom(\mu)$, $\mu(?X) \in O$, $\mu(?Y) \in O$, and $\mu(?X) = \mu(?Y)$;
\item 
$C$ is ${label(?X)} = {p}$, $?X \in \dom(\mu)$, $\mu(?X) \in O$, and $\lab(?X) = p$; 
\item 
$C$ is ${label(?X)} = {label(?Y)}$, $?X \in \dom(\mu)$, $?Y \in \dom(\mu)$, $\mu(?X) \in O$, $\mu(?Y) \in O$, and $\lab(?X) = \lab(?Y)$; 
\item 
$C$ is ${?X.p} = {?Y.q}$, $?X \in \dom(\mu)$, $?Y \in \dom(\mu)$, $\mu(?X) \in O$, $\mu(?Y) \in O$ and $\prop(\mu(?X),p) = \prop(\mu(?Y),q)$;
\item 
$C$ is ${?X.p} = {a}$, $?X \in \dom(\mu)$, $\mu(?X) \in O$ and $\prop(\mu(?X),p) = a$;
\item
$C$ is $(C_1 \land C_2)$, $C_1$ and $C_2$ are selection conditions, $\mu \models_G C_1$ and $\mu \models_G C_2$; 
\item
$C$ is $(C_1 \lor C_2)$, $C_1$ and $C_2$ are selection conditions, $\mu \models_G C_1$ or $\mu \models_G C_2$; 
\item
$C$ is $(\neg C_1)$, $C_1$ is a selection condition, and it is not the case that $\mu \models_G C_1$. 
\end{itemize}

The evaluation of a graph pattern $P$ over a property domain graph $G=(O,\gamma,\lab,\prop)$, is defined as a function $\semp{P}{G}$ which returns a set of solution mappings. 
If $P$ is a simple pattern $(t_1, t_2, t_3)$ then 
\begin{verse}
$\semp{P}{G} = \{ \mu \mid \dom(\mu) = var(P) ~\land~ \gamma(\mu(t_2)) = (\mu(t_1), \mu(t_3)) \}$  
\end{verse}
where $var(P)$ is the set of variables occurring in $P$.
The semantics of complex graph patterns is defined as follows:
\begin{verse}
$\semp{(P_1 \AAND P_2)}{G} = \semp{P_1}{G} \Join \semp{P_2}{G}$

$\semp{(P_1 \OPT P_2)}{G} = \semp{P_1}{G} \LOJ \semp{P_2}{G}$
\end{verse}

Given a domain graph $G=(O,\gamma,\lab,\prop)$, a path in $G$ is a sequence $ S = [o_1, \dots, o_n] $ where $o_1, \dots, o_n \in \objs$, and satisfying that for each pair $(o_i, o_{i+1})$ with $1 \leq i < n$, it applies that $\gamma(o_i) = (a,b)$ and $\gamma(o_{i+1})=(b,c)$. The length of $S$, denoted as $length(S)$, is $n$. 






















==> sections/langabstract.tex <==
In this subsection, we give an abstract characterization of queries in MillenniumDB, and formally define their semantics. Following this, we will map the concrete syntax used by MilleniumDB to this abstract specification. Formally, let $\vars$ be an infinite set $\{\texttt{?x}, \texttt{?y}, \ldots\}$ of \emph{variables}, disjoint from $\objs$. The general shape of a query in MilleniumDB can be specified as:

\begin{tabular}{l}
\texttt{SELECT}\ \texttt{Selectors}\\
\texttt{MATCH}\ \texttt{MatchPattern}\\
\texttt{FILTER}\ \texttt{Filters}
\end{tabular}

The main work is done in the \texttt{MatchPattern}, which specifies a subgraph we are looking for in the property-domain graph. The set of \texttt{MatchPattern}s can be defined recursively as follows:
\begin{itemize}
\item \texttt{($v$ $l_1\cdots l_m$ \{$k_1:v_1,\ldots ,k_n:v_n$\})}, with $v\in \vars \cup \objs, l_1,\ldots ,l_m \in \labels, k_1\ldots, k_n\in \keys$, and, $v_1,\ldots ,v_n\in\values$, is a \texttt{MatchPattern} called a \texttt{NodePattern}
\item \texttt{nP$_1$-[$e$ $t$ \{$k_1:v_1,\ldots ,k_n:v_n$\}]->nP$_2$}, where \texttt{nP$_1$, nP$_2$} are \texttt{NodePattern}s, $e\in \vars$, $t\in \objs \cup \vars, k_1\ldots, k_n\in \keys$, and, $v_1,\ldots ,v_n\in\values$, is a \texttt{MatchPattern} called an \texttt{EdgePattern}
\item \texttt{nP$_1$=[pathExp]=>nP$_2$}, where $k_1\ldots, k_n\in \keys$, and, \texttt{pathExp}  a path expression as defined below, is a \texttt{MatchPattern} called a \texttt{PropertyPath}
\item If \texttt{P$_1$} and \texttt{P$_2$} are \texttt{MathExpression}, then \texttt{(P$_1$ JOIN P$_2$)} is a  \texttt{MathExpression}, called a \texttt{BasePattern}
\item If \texttt{P$_1$} and \texttt{P$_2$} are \texttt{MathExpression}, then \texttt{(P$_1$ OPTIONAL P$_2$)} is \texttt{MathExpression}, called an \texttt{OptionalExpression}.
\end{itemize}

A \texttt{pathExp} \texttt{e} is defined by the following grammar:
$$\texttt{e} :-\ o \ |\ \hat{ } o \ |\ (\texttt{e}_1\slash \texttt{e}_2) \ |\ (\texttt{e}_1 + \texttt{e}_2) \ |\ \texttt{e}^* \ |\ \texttt{e}?$$
where $\texttt{e},\texttt{e}_1,\texttt{e}_2$ are \texttt{pathExp}, and $o\in \objs$.

The \texttt{Selectors} are simply a set of expressions of the form 
$\texttt{?x}$ and \texttt{?x}.k, where $\texttt{?x}\in \vars$, and $k\in \keys$, or the symbol $*$.

Finally, the \texttt{Filters} \texttt{f} is given by the grammar:
$$
\texttt{f} :-\ \texttt{?x}.k\sim val \ |\ \texttt{?x}.k\sim \texttt{?y}.k' \ |\ (\texttt{f}_1 \ \texttt{AND}\ \texttt{f}_2) \ |\ (\texttt{f}_1 \ \texttt{OR}\ \texttt{f}_2)
$$
where $\texttt{f}, \texttt{f}_1$ and $\texttt{f}_2$ are \texttt{Filters}, $\texttt{?x}, \texttt{?y}\in \vars, val\in \values, k,k'\in \keys$, and $\sim \in \{\texttt{==,<,>,<=,>=}\}$.

If $q$ is a query, $\vars(q)$ denotes the set of its variables, that is, the set of all elements $v\in \vars$ that appear in the \texttt{MatchPattern} of $q$. Notice here that in each \texttt{NodePattern} we can have at most one variable identifying the node, or its explicit identifier. Similarly, for each \texttt{PropertyPath}, we can have at most two variables,  corresponding to the end nodes of the path. In the case of \texttt{EdgePattern}, we can have at most four variables. Two of these correspond to the end nodes of the edge, and the other two to the edge identifier, and its type. For a query to be syntactically correct, we require that each variable appearing in \texttt{Selectors}, and each variable appearing in \texttt{Filters}, also appears in \texttt{MatchPattern}.

The semantics of a query $q$ over a property-domain graph $G$ is defined in terms of mappings, analogously to SPARQL \cite{PerezAG09}, or to homomorphism based semantics of property graphs \cite{AnglesABHRV17}. A \textit{mapping} is a partial function $\mu: \vars \mapsto \objs$. The \emph{domain} $\Dom{\map}$ of a mapping $\map$ is the set of variables on which $\map$ is defined. Additionally, we will assume that $\mu(o)=o$, for all $o\in \objs$. We will write $\mu_{|\mathcal{X}}$ to denote the restriction of $\mu$ to the set of variables $\mathcal{X}$. Two mappings $\map_1$ and $\map_2$ are \emph{compatible} (written as $\map_1 \sim \map_2$) 
if $\map_1(?x) = \map_2(?x)$ for all variables $?x$ which are in both $\Dom{\map_1}$ and $\Dom{\map_2}$. 
If $\map_1 \sim \map_2$, then 
we write $\map_1 \cup \map_2$ for the mapping obtained 
by extending $\map_1$ according to $\map_2$ on all the variables in $\Dom{\mu_2}\setminus\Dom{\mu_1}$. Given two sets of mappings $\mset_1$ and $\mset_2$, 
the \emph{join}, \emph{difference} and \emph{left outer join} between $\mset_1$ and $\mset_2$ are defined respectively as follows:
$$
\begin{array}{ccl}
\mset_1 \Join \mset_2 & = & \{\map_1 \cup \map_2 \mid \map_1 \in \mset_1,  \map_2 \in \mset_2, 
 \text{ and } \map_1 \sim \map_2\} \\
%\mset_1 \cup \mset_2 & = & \{\map \mid \map \in \mset_1 \text{ or } \map \in \mset_2\}, \\
\mset_1 \setminus \mset_2 & = & \{\map_1 \mid \map_1 \in \mset_1,   \text{ and } \forall \map_2 \in \mset_2, \map_1 \nsim \map_2\}\\
\mset_1 \LOJ \mset_2 & = & (\mset_1 \Join \mset_2) \cup (\mset_1 \setminus \mset_2)

\end{array}
$$


\begin{figure}
$\begin{array}{rcl}
\semp{\texttt{:}o}{G} & = & \{(o_1,o_2) \mid \gamma(o') = (o_1,o,o_2), \text{ for some }o'\in O\}, \\
\semp{\hat{ }\ e}{G} & = & \{(o_1,o_2) \mid (o_2,o_1)\in \semp{e}{G}\}, \\
\semp{e_1 \slash e_2}{G} & = & \semp{e_1}{G}\circ \semp{e_2}{G}, \\
\semp{e_1 | e_2}{G} & = & \semp{e_1}{G}\cup \semp{e_2}{G}, \\
\semp{e^+}{G} & = & \bigcup_{k\geq 1} \semp{e}{G}^k, \\
\semp{e^*}{G} & = & \{(o,o) \mid o\in O\} \cup \semp{e^+}{G}, \\
\semp{e?}{G} & = & \semp{e}{G} \cup \{(o,o) \mid o\in O\}. \\
\end{array}$
\caption{Semantics of \texttt{pathExp} over a domain-graph $G = (O,\gamma)$. Here $e,e_1,e_2$ stand for any \texttt{pathExp}.}
\label{fig-pathexp}
\end{figure}


Let $q$ be any MillenniumDB query. To define its semantics over a property-domain graph $G=(O,\gamma,\texttt{lab},\texttt{prop})$, we first define the set of mappings that belong to the evaluation of its \texttt{MatchPattern} $\texttt{MP}(q)$, denoted by $\semp{\texttt{MP}(q)}{G}$. We can define $\semp{\texttt{MP}(q)}{G}$ inductively as follows:

\begin{itemize}
\item If $\texttt{MP}(q)$ \texttt{:- ($v$ $l_1\cdots l_m$ \{$k_1:v_1,\ldots ,k_n:v_n$\})}, then the set  $\semp{\texttt{MP}(q)}{G}$ contains all mappings $\mu:\vars(q)\mapsto \objs$, such that:
\begin{itemize}
\item $\mu(v)\in O$,
\item $\{l_1,\ldots, l_m\} \subseteq \lab(\mu(v))$, and
\item $\prop(\mu(v),k_i) = v_i$, for $i=1\ldots n$.
\end{itemize}
Notice that $\semp{\texttt{MP}(q)}{G} = \{\mu_{\emptyset}\}$  whenever $v = o\in \objs$, the node $o$ is present in the database, and has the appropriate labels and properties. Here $\mu_{\emptyset}$ denotes the empty mapping.
\item If $\texttt{MP}(q)$ \texttt{:- nP$_1$-[$e$ $t$ \{$k_1:v_1,\ldots ,k_n:v_n$\}]->nP$_2$}, then $\semp{\texttt{MP}(q)}{G}$ contains all mappings $\mu:\vars(q)\mapsto \objs$ where:
\begin{itemize}
\item $\mu_{|\qvars{\texttt{nP}_1}} \in \semp{\texttt{nP}_1}{G}$,
\item $\mu_{|\qvars{\texttt{nP}_2}} \in \semp{\texttt{nP}_2}{G}$,
\item $\gamma(\mu(e)) = (\mu(v^{\texttt{nP}_1}),\mu(t),\mu(\mu(v^{\texttt{nP}_1}))$, and
\item $\prop(\mu(e),k_i) = v_i$, for $i=1\ldots n$.
\end{itemize}
\item If $\texttt{MP}(q)$ \texttt{:- nP$_1$=[pathExp]=>nP$_2$}, then $\semp{\texttt{MP}(q)}{G}$ contains all mappings $\mu:\qvars{q}\mapsto \objs$ where:
\begin{itemize}
\item $(\mu(v^{\texttt{nP}_1}),\mu(v^{\texttt{nP}_1})) \in \semp{\texttt{pathExp}}{G}$, with $\semp{\texttt{pathExp}}{G}$ as defined in Figure \ref{fig-pathexp}.
\end{itemize}
\item If  $\texttt{MP}(q)$ \texttt{:- (P$_1$ JOIN P$_2$)}, then
 $$\semp{\texttt{MP}(q)}{G} = \semp{\texttt{P}_1}{G} \Join \semp{\texttt{P}_2}{G}$$
\item If  $\texttt{MP}(q)$ \texttt{:- (P$_1$ OPTIONAL P$_2$)}, then
 $$\semp{\texttt{MP}(q)}{G} = \semp{\texttt{P}_1}{G} \LOJ \semp{\texttt{P}_2}{G}$$
\end{itemize}

In order to define the semantics of the of the entire query, we next need to define when a mapping $\mu$ satisfies a \texttt{Filter} \texttt{f} over a property-domain graph $G=(O,\gamma,\texttt{lab},\texttt{prop})$, denoted as $G,\mu \models \texttt{f}$. This is again done inductively on the structure of \texttt{f}:
\begin{itemize}
\item $G,\mu \models \texttt{?x}.k \sim val \Leftrightarrow \texttt{prop}(\mu(\texttt{?x}),k) \sim val$
\item $G,\mu \models \texttt{?y}.k' \sim val \Leftrightarrow \texttt{prop}(\mu(\texttt{?x}),k) \sim \texttt{prop}(\mu(\texttt{?x}),k)$
\item $G,\mu \models (\texttt{f}_1 \ \texttt{AND}\ \texttt{f}_2) \Leftrightarrow G,\mu \models \texttt{f}_1 \text{ and } G,\mu \models \texttt{f}_2$
\item $G,\mu \models (\texttt{f}_1 \ \texttt{OR}\ \texttt{f}_2) \Leftrightarrow G,\mu \models \texttt{f}_1 \text{ or } G,\mu \models \texttt{f}_2$.
\end{itemize}

Finally, if $q$ is a query of the form

\begin{tabular}{l}
\texttt{SELECT}\ \texttt{Selectors}\\
\texttt{MATCH}\ \texttt{MatchPattern}\\
\texttt{FILTER}\ \texttt{Filters}
\end{tabular}
then we can define the evaluation of $q$ over a property-domain graph $G=(O,\gamma,\texttt{lab},\texttt{prop})$, denoted $\eval{q}{G}$ as follows:
\begin{itemize}
\item If \texttt{Selectors = $*$}, then:
$$\eval{q}{G} = \{\mu \ \mid \ \mu \in \semp{\texttt{MP}(q)}{G}, \text{ and } G,\mu \models \texttt{Filters}\}.$$
\item If \texttt{Selectors = }$\mathbf{V} \cup \mathbf{KV}$, where $\mathbf{V}\subseteq \vars(q)$, and each $\texttt{?x}.k\in \mathbf{KV}$ is such that $\texttt{?x}\in \vars(q)$ and $k\in \keys$, then let $\texttt{SelVars(q)}$ denote the set of all variables $\texttt{?x}$ such that $\texttt{?x}\in \mathbf{V}$, or $\texttt{?x}.k\in \mathbf{KV}$, for some $k\in \keys$. We define the set $\eval{q}{G}$ to consist of all mappings $\texttt{res}:\mathbf{V}\cup \mathbf{KV}\mapsto \objs \cup \values$, such that there exists $\mu \in \semp{\texttt{MP}(q)}{G}$ with:
\begin{itemize}
\item $\mu_{|\texttt{SelVars(q)}} = \texttt{res}_{|\texttt{SelVars(q)}}$;
\item $G,\mu \models \texttt{Filters}$; and
\item $\texttt{res}(\texttt{?x}.k) = \texttt{prop}(\mu(\texttt{?x}),k)$, for each $\texttt{?x}.k \in \mathbf{KV}$. Whenever $\texttt{prop}(\mu(\texttt{?x}),k)$, we assume this value to be equal to the constant \texttt{NULL}.
\end{itemize}
\end{itemize}


==> sections/planner.tex <==
The query execution pipeline follows the standard database template:
\begin{itemize}
\item The string of the query is parsed into an Abstract Syntax Tree (AST), and checked that it complies with the grammar specified in Figure \ref{fig-syntax}.
\item A logical plan is generated using a depth-first traversal of the AST, instantiating nodes of the tree to logical operators (e.g. there will be nodes corresponding to the MATCH, FILTER, or any other clause in the query). Logical operators have Op prefixed to their name, and will thus be called OpMatch, OpSelect, etc.
\item Using a visitor-pattern \cite{}, the logical tree is parsed in order to apply some basic simplifications (e.g. pushing constant from filters into the search pattern)\footnote{At this point MillenniumDB does not have a fully developed query rewriting module which would naturally fit here. This is left as future work.}.
\item Finally, another pass of the logical tree using the visitor-pattern is made in order to create a physical plan.
\end{itemize}

An illustration of what a logical plan looks like for a generic MillenniumDB query is given in Figure \ref{fig-logical}. Here each \texttt{OpMatch} is also associated with the BGPs and property paths appearing in it, but we omit those for brevity. As we can notice, some parts of the query are mandatory (corresponding to the SELECT and MATCH clauses), while the other need not be present.

\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
\begin{lstlisting}
SELECT SelOptions
MATCH  MatchPattern
WHERE  Condition
\end{lstlisting}
\end{minipage}%

\begin{minipage}{.45\columnwidth}
  \centering
\begin{tikzpicture}
%\node[iri,right=\hgap of sp1] (ch1) {$v_3$}
%  edge[arrin,bend right=20] node[var] (e1) {$v_1$ : P39} (sp1)
%  edge[arrin,bend left=20] node[var] (e2) {$v_2$ : P39} (sp1);

\node[fill=red!20, draw, rounded corners] (Sel) {$\texttt{OpSelect}$};

\node[below = 0.6cm of Sel, fill=yellow!20, draw, rounded corners] (Fil) {$\texttt{OpFilter}$};

\node[below = 0.6cm of Fil, fill=red!20, draw, rounded corners] (Root) {$\texttt{OpGraphRoot}$};

\node[below = 0.6cm of Root, fill=blue!20, draw, rounded corners] (Pat) {$\texttt{GraphPattern}$};

\draw[<-,thick, color = red] (Sel)--(Fil);
\draw[<-,thick, color = red] (Fil)--(Root);
\draw[<-,thick, color = red] (Root)--(Pat);
\end{tikzpicture}
\end{minipage}%
\begin{minipage}{.45\columnwidth}
  \centering
\begin{tikzpicture}

\node[] (GP) {$\texttt{GraphPattern}$};

\node[below = 0.5cm of GP, fill=red!20, draw, rounded corners] (M) {$\texttt{OpMatch}$};

\node[below = 0.3cm of M] (tt) {Or:};

\node[below = 0.3cm of tt, fill=red!20, draw, rounded corners] (OP) {$\texttt{OpOptional}$};

\node[below left = 0.5cm and -0.3cm of OP, fill=red!20, draw, rounded corners] (M1) {$\texttt{OpMatch}$};

\node[right = 0.4cm of M1, fill=blue!20, draw, rounded corners] (O1) {$\texttt{GraphPattern}$};



\draw[<-,thick, color = red] (OP)--(M1);
\draw[<-,thick, color = red] (OP)--(O1);
%\draw[<-,thick, color = red] (Root)--(Pat);
\end{tikzpicture}
\end{minipage}%
\caption{A logical plan for a generic MillenniumDB query. Red and blue nodes must always be present in the query plan, while the yellow ones are not always specified. Graph pattern is either a single conjunction of atomic patterns (node, edge, or property path patterns), or an OPTIONAL pattern.}
\label{fig-logical}
\end{figure}

The most interesting aspect of query execution happens in generating the physical plan. The general structure is quite simple: each \texttt{Op} node in the logical plan is assigned a linear iterator returning solution mappings, and can pass its results to the node above following the red arrows in Figure \ref{fig-logical}. The interesting part is evaluating each \texttt{OpMatch} pattern, which consists of a conjunction of basic graph patterns and property paths. In essence, evaluating BGPs is analogous to selecting an appropriate join plan for the relations representing the different elements of BGPs (e.g. node labels, key values, connections, etc.). This also goes in hand with selecting the appropriate join algorithm for each of the joins. Given that the relations used in BGPs are all indexed, this will most commonly be index nested loops join. Property paths on the other hand require an entirely different set of techniques for their evaluation, and are currently pushed to the very end of query execution and joined via a nested-loop join with the remaining BGPs \footnote{We admit that this is not always the best option. However, based on extensive empirical evidence (see the experiments in Section \ref{sec:benchmark}), this solution is more than adequate in practice.}. We illustrate a sample query, and a possible plan generated for this query in Figure \ref{fig-phys}.

\begin{figure}
\begin{minipage}{.65\columnwidth}
  \centering
\begin{lstlisting}
SELECT ?x, ?y
MATCH (?x :Person)-[:knows]->(?y :Person)
\end{lstlisting}
\end{minipage}%

\begin{minipage}{.45\columnwidth}
  \centering
\begin{tikzpicture}
\node[fill=red!20, draw, rounded corners] (Sel) {$\texttt{OpSelect}$};

\node[below = 0.6cm of Sel, fill=red!20, draw, rounded corners] (Root) {$\texttt{OpGraphRoot}$};

\node[below = 0.8cm of Root, fill=blue!10, draw, rounded corners, dashed] (Pat) {
   \alt{ \\
        \texttt{OpLabel(?x, Person)}\\
        \texttt{OpLabel(?y, Person)}\\
        \texttt{OpConnection(?x, ?\_e, knows, ?y)}}  };
         
\node[fill=blue!20, draw, rounded corners] (le1) at (Pat.north) {$\texttt{OpMatch}$};

\draw[<-,thick, color = red] (Sel)--(Root);
\draw[<-,thick, color = red] (Root)--(le1);
\end{tikzpicture}
\end{minipage}%

\resizebox{\columnwidth}{!}{
\includegraphics[scale=1.0]{./images/plan.png}
}

\caption{Generating a physical plan based on a logical plan. Notice that the \texttt{OpMatch} now lists the relations that are to be joined in the query, and an implicit edge variable \texttt{?\_e} is introduced. The physical plan in this case simply joins the used relations.}
\label{fig-phys}
\end{figure}

Currently, MillenniumDB supports three different evaluation mechanisms for evaluating BGPs and property paths:
\begin{itemize}
\item The classical relational optimizer which is based on cost estimation, and tries to order base relations in such a way as to minimize the amount of (intermediate) results. We currently support two modes of execution here:
\begin{itemize}
\item[(i)] Selinger-style join plans \cite{Sciore20} which use dynamic programming to determine the optimal order of BGPs.
\item[(ii)] In the presence of a large number of BGPs, a greedy planner \cite{0020812} is used which simply determines the cheapest relation to use in each step.
\end{itemize}
\item A worst-case optimal query plan as described in \cite{HoganRRS19} is used whenever possible. This approach implements a modified leapfrog algorithm of \cite{Veldhuizen14} in order to minimize the number of intermediate results that are generated.
\item For property paths, a modified breadth-first search algorithm is used as proposed in \cite{BaierDRV17}.
\end{itemize}

Two points of interest in the way that MillenniumDB handles query execution are the worst-case optimal query planner for BGPs, and the way that property paths are handled, given that that these differ from the usual evaluation techniques somewhat. We provide some additional details on these next.

Evaluating BGPs in a worst-case optimal way is done using a modified leapfrog algorithm \cite{Veldhuizen14}, similarly as in \cite{HoganRRS19}. For this...TODO

Finally, the heuristic we deploy for selecting the variable ordering used in our implementation of the leapfrog algorithm mixes the greedy approach and the ideas of the GYO reduction \cite{YuO79}. More precisely, we first order the variables based on the minimal cost of the relations they appear in, and resolve ties by selecting the variable that appears in more distinct relations participating in the join. The variables ``connected" to the first one selected are then processed in the same manner (where connected meant appearing in the same relation), until the process can not continue. The isolated variables are then treated last.

On the other hand, property paths are evaluated via a breadth-search algorithm\footnote{BFS is the default evaluation method for property paths. The source code also includes four other algorithms, each with their merits and cons. Detailed exploration of those is outside of the scope of this paper.} adopted to property paths \cite{BaierDRV17}. Our assumption is that each property path pattern will have at least one of the endpoints assigned before evaluation. This can be done either explicitly in the pattern, or via the remainder of the query. For instance, a property paths pattern \texttt{(Q1)=[:P31*]=>(?x)} has the starting point of our search assigned to \texttt{Q1}. On the other hand, \texttt{(?x)=[:P31*]=>(?y), (?y :Person)} does not have any of the endpoints assigned, however, the \texttt{(?y :Person)} allows us to instantiate \texttt{?y} with any node with the label \texttt{:Person}.

For evaluating a property path, the path pattern is then compiled into an automaton, and a ``virtual" cross-product of this automaton and the graph is constructed and navigated in a breadth-first manner. Intuitively, from a starting node (tagged with the initial state of the query automaton), all connections with they type specified by the outgoing transitions from this state are followed. The process is repeated until reaching an end state of the automaton, upon which, a result can be returned. This allows a fully pipelined evaluation of property paths, and additionally requires to have at most one page pinned in the buffer on execution (the neighbors of the node on the top of the BFS queue).

 Additionally, the BFS algorithm also allows us to return a single shortest path between each pair of endpoints. We allow specifying this by adding a variable in the property path pattern as follows:
\begin{lstlisting}
SELECT *
MATCH (Kevin Bacon)=[?p (:actedIn/^:actedIn)*]=>(?actor)
\end{lstlisting} 
\riveros{The use of variables in the pattern is not mentioned in the query language, isn't it?}
Intuitively, this query anchors the search at the node corresponding to \texttt{Kevin Bacon}, and looks for all the actors who acted with him in the same movie, or in a movie with someone who acted with him, etc. The variable \texttt{?p} will return a single shortest path between Kevin Bacon and any other actor who can be reached via a path satisfying the query. We note that returning path comes basically for free, given that they can be reconstructed using the set of visited nodes which is used for bookkeeping in the BFS algorithm.






==> sections/semantics.tex <==
%!TEX root = ../main.tex

\subsection{Semantics of Domain Graph Queries}

%Based on our domain graph model,
Queries in MillenniumDB are
%also
based on an abstract notion of \textit{domain graph query}, which
%that
generalise the types of graph patterns used
%popularised
by modern graph query languages~\cite{AnglesABHRV17}. This query
abstraction provides modularity in terms of how the database is
constructed, flexibility in terms of what concrete query syntax is
supported, and allows for defining its semantics and studying its
theoretical properties in a clean way.

This section provides an overview of the formal definition of the
MillenniumDB query language
%i.e. its abstract syntax and semantics.
(its complete definition can be found in Appendix
\ref{sec-app-semantics}). From now on, assume a countably infinite
set $\vars$ of variables disjoint with the set of objects $\objs$.


%-----------
\textbf{Basic graph patterns.} At the core of domain queries are basic graph patterns.\footnote{Basic graph patterns correspond to conjunctive queries (CQs) over graphs.} 
%\ah{How about changing $\vars$ to $\mathcal{V}$ to look like $\objs$. Or maybe $\objs$ to \textsf{Objs} (though I guess the former is more concise?) :)} \dv{Sure, go ahead. Left it as a macro for that reason.} %ah: done
A \emph{basic graph pattern} is defined as a pair $(V,\phi)$ such that $\phi : (\objs \cup \vars) \rightarrow (\objs \cup \vars) \times (\objs \cup \vars) \times (\objs \cup \vars)$ is a partial mapping with a finite domain and $V \subseteq \Var{\phi}$, where $\Var{\phi}$ is the set of variables occurring in the domain or in the range of $\phi$. Thus, $\phi$ can be thought of as a domain graph that allows a variable in any position, together with a set $V$ of output variables (hence the restriction that each variable in $V$ occurs in $\phi$).

The evaluation of a basic graph pattern returns a set of solution
mappings.  A \textit{solution mapping} (or simply \textit{mapping}) is
a partial function $\map: \vars \rightarrow \objs$. 
The \emph{domain} of a mapping $\map$, denoted by $\Dom{\map}$, is the set of variables on which $\map$ is defined. 
Given $v \in \vars$ and $o \in \objs$, we use $\mu(v) = o$ to denote that $\mu$ maps variable $v$ to object $o$. 
Besides, given a set $V$ of variables, the term $\mu_{|_V}$ is used to denote the mapping obtained by restricting $\mu$ to $V$, that is, $\mu_{|_V} :
(V \cap \Dom{\mu}) \to \objs$ such that $\mu_{|_V}(v) = \mu(v)$ for every $v \in (V \cap \Dom{\mu})$ (notice that $V$ is not assumed to be subset of $\Dom{\mu}$).
Finally, for the sake of presentation, we assume that $\mu(o)=o$, for
all $o\in \objs$.

The evaluation of a basic graph pattern $B = (V,\phi)$ over a property-domain graph 
$G=(O,\gamma)$, denoted by $\semp{B}{G}$, is defined as
%follows:
%The semantics of $\semp{P}{G}$ is given as follows:
%\begin{eqnarray*}
  $\semp{B}{G} = \{ \map_{|_V} \mid \mu \in \semp{\phi}{G}\}$,
%\end{eqnarray*}
where 
\begin{multline*}
  \semp{\phi}{G} \ = \ \{ \map \mid
  \Dom{\map} = \Var{\phi} \text{ and if } \phi(a) = (a_1,a_2,a_3),\\ 
  \text{then } \gamma(\map(a)) = ( \map(a_1), \map(a_2), \map(a_3)  ) \}.
\end{multline*}
%\color{black}
For example, consider the basic graph pattern $(V,\phi)$ where $V = \{ v_2, v_4, v_6\}$ and $\phi$ is given by the assignments:
\begin{verse} 
$\phi(v_1) = (v_2, \texttt{position held}, \texttt{President of Chile})$,\\
$\phi(v_3) = (v_1, \texttt{start date}, v_4)$, and\\
$\phi(v_5) = (v_1, \texttt{replaces}, v_6)$.
\end{verse}
In Figure \ref{fig:bgp}, we provide a graphical representation of the above graph pattern, and the solution mappings obtained by evaluating the graph pattern over the property domain graph shown in Figure~\ref{fig:dg2}. The solution mappings are presented as a table with columns $v_2$, $v_4$, $v_6$ (i.e. the variables in $V$), and each row represents an individual mapping. Per our definitions, different variables may map to the same object in a single solution. Thus, our notion of evaluation follows a homomorphism-based semantics, similar to query languages such as SPARQL~\cite{AnglesABHRV17}.\footnote{Isomorphism-based semantics~\cite{AnglesABHRV17} -- such as Cypher's no-repeated-edge semantics, which disallows the same solution to use the same edge twice -- can be emulated by filtering solutions after they are generated.}

\begin{figure}[tb]
\setlength{\vgap}{1.2cm}
\setlength{\hgap}{4cm}
\centering

\begin{tikzpicture}

\node[iri,anchor=center,minimum width=7.5cm,minimum height=0.7cm,dashed] (e1) {};

\node[anchor=south east,above left=0.1ex of e1.south east] (e1i) {$v_1$};

\node[iri,right=1ex of e1.west,anchor=west] (sp1) {$v_2$};
\node[iri,right=\hgap of sp1] (ch1) {President of Chile}
  edge[arrin] node[iri,draw=none] {position held} (sp1);
  
\node[iri,below=\vgap of sp1] (v4) {$v_4$}
  edge[arrin] node[lab] {start date} (e1);

\node[iri,below=\vgap of ch1] (mb) {$v_6$}
  edge[arrin] node[lab,xshift=-1ex] {replaces} (e1);
  
\end{tikzpicture}

\medskip

\begin{tabular}{lllllll}
\toprule
$v_2$ & $v_4$ & $v_6$ \\
\midrule
\texttt{Michelle bachelet} & \texttt{2006-03-11} & \texttt{Ricardo Lagos} \\
\texttt{Michelle bachelet} & \texttt{2018-03-11} & \texttt{Sebastián Piñera}\\ 
\bottomrule
\end{tabular}

\caption{Graphical representation of a basic graph pattern (top), and the tabular representation of the solution mappings (bottom) obtained by evaluating the basic graph pattern
%after the evaluation
  over the property domain graph shown in Figure~\ref{fig:dg2} \label{fig:bgp}.}
\end{figure}

%-----------
\textbf{Navigational graph patterns.}
A characteristic feature of graph query languages is the ability to match paths of arbitrary length that satisfy certain criteria. We call basic graph patterns enhanced with this feature \textit{navigational graph patterns}, and we define them next.

A popular way to express criteria that paths should match is through regular expressions on their labels, aka.\ \textit{regular path queries} (\textit{rpqs}). More precisely, an \textit{rpq expression} $r$ is defined by the following grammar:
\begin{eqnarray*}
  r & ::= & \varepsilon \ \mid \ o \in \objs \ \mid \  (r/r) \ \mid \ (r + r) \ \mid \ \inv{r} \ \mid \ r^*.
\end{eqnarray*}
%where $\texttt{e},\texttt{e}_1,\texttt{e}_2$ are rpq expressions, and $o\in \objs$.
The semantics of an rpq expression $r$ is defined in terms of its
evaluation on a property-domain graph $G$, denoted by $\semp{r}{G}$, which
returns a set of pair of nodes in the graph that are connected by
paths satisfying $r$. More precisely, assuming that $G = (O,\gamma)$,
$o \in \objs$ and $r,r_1,r_2$ are rpq expressions, we have that:
\begin{eqnarray*}
\semp{\varepsilon}{G} & = & \{(o,o) \mid o\in O\},\\
\semp{o}{G} & = & \{(o_1,o_2) \mid \exists o' \in \objs : \gamma(o') = (o_1,o,o_2)\},\\
\semp{(r_1 / r_2)}{G} & = & \{ (o_1,o_2) \mid \exists o' \in \objs : (o_1,o') \in \semp{r_1}{G} \text{ and}\\
&& \phantom{\{ (o_1,o_2) \mid} (o',o_2) \in \semp{r_2}{G}\}, \\
\semp{(r_1 + r_2)}{G} & = & \semp{r_1}{G}\cup \semp{r_2}{G}, \\
\semp{\inv{r}}{G} & = & \{(o_1,o_2) \mid (o_2,o_1)\in \semp{r}{G}\}.
\end{eqnarray*}
Moreover, assuming that $r^1 = r$ and $r^{n+1} = r/r^n$ for every $n \geq 1$, we have that:
\begin{eqnarray*}
  \semp{r^*}{G} & = & \semp{\varepsilon}{G} \, \cup \, \bigcup_{k \geq 1} \semp{r^k}{G}.
\end{eqnarray*}
Other rpq expressions widely used in practice can be defined by
combining the previous operators. 
In particular, we have that $r? = \varepsilon + r$ and $r^+ = r/r^*$.

%Basic graph patterns can then be extended in a natural way in order to allow rpqs to capture paths over multiple graphs. \ah{Well maybe not so natural as we have to deal with edge ids for rpqs, which, when a variable, should probably return a sequence of edge ids I guess (a complex object)? This might then lead to infinite graphs, so the would need to be given under some restricted semantics (simple paths, or whatever). Or maybe they could just be projected away. Anyways, postponing this for now. :)}

An \textit{path pattern} is a tuple $(a_1,r,a_2)$ such that $a_1, a_2 \in \objs \cup \vars$ and $r$ is an rpq expression. 
As for the case of basic graph patterns, given a path pattern $p$, we use the term $\Var{p}$ to denote the set of variables occurring in $p$. 
Moreover, the evaluation of $p = (a_1,r,a_2)$ over a property-domain graph $G$, denoted by $\semp{p}{G}$, is defined as:
\begin{eqnarray*}
  \semp{p}{G} &=& \{ \mu \mid \Dom{\mu} = \Var{p} \text{ and } (\mu(a_1),\mu(a_2)) \in \semp{r}{G} \}.
\end{eqnarray*}

For example, the expression ( \texttt{Michelle Bachelet}, \texttt{replaced by}$^+$, $v$) is a path pattern that returns all the Presidents of Chile after Michelle Bachelet.  

Given a set $\psi$ of path patterns, $\Var{\psi}$ also denotes the set of variables occurring in $\psi$, and the evaluation of $\psi$ over a property-domain graph $G$ is defined as:
\begin{multline*}
  \semp{\psi}{G} \ = \ \{ \mu \mid \Dom{\mu} = \Var{\psi} \text{ and}\\ \mu_{|_{\Var{p}}} \in \semp{p}{G} \text{ for each } p \in \psi \}.
\end{multline*}

\begin{definition}
A \emph{navigational graph pattern} is a triple $(V,\phi,\psi)$ where $(V' \subseteq V, \phi)$ is a basic graph pattern, $\psi$ is a set of path patterns and $V \subseteq \Var{\phi} \cup \Var{\psi}$. 
The semantics of a navigational graph pattern $N = (V,\phi,\psi)$ is defined as:
\begin{multline*}
   \semp{N}{G} \ = \ \{ \mu_{|_V} \mid \Var{\mu} = \Var{\phi} \cup \Var{\psi},\\ \mu_{|_{\Var{\phi}}} \in \semp{\phi}{G} \ \text{ and } \ 
    \mu_{|_{\Var{\psi}}} \in \semp{\psi}{G} \}. \qed
  \end{multline*}
\end{definition}
Hence, the result of a navigational graph pattern $N = (V,\phi,\psi)$ is a set of mappings $\mu$ projected onto the set $V$ of output variables, where $\mu$ satisfies the structural restrictions imposed by $\phi$ and the path constrainst imposed by $\psi$.
Notice that multiple rpq expressions can link the same pair of nodes. This is similar to the existential semantics of path queries, as specified in the SPARQL standard \cite{HarrisS13}.

Given a domain graph $G=(O,\gamma,\lab,\prop)$, currently we define paths over the directed edge-labelled graph that forms the range of $\gamma$; in other words, we do not allow for matching paths that emanate from an edge object. Such a feature could be considered in the future. We may also consider adding semantics for shortest paths, additional criteria on node or edges in the path, etc.

%\dv{We can actually talk about returning paths here. From a practical perspective, we could specify that each rpq returns a lexicographically smallest shortest path. This is currently done by the BFS implementation (well not really, but can be tweaked to do this). Another option would be to return all shortest paths. Again, BFS style algorithms can do this in practice.}

%-----------
\textbf{Relational graph patterns.}
As previously discussed (and seen in the example of Figure~\ref{fig:bgp}), graph patterns return relations (tables) as solutions. Thus we can -- and many practical graph query languages do -- use a relational-style algebra to transform and/or combine one or more sets of solution mappings into a final result.  

Towards defining this algebra, we need the following terminology.
Two mappings $\map_1$ and $\map_2$ are \emph{compatible}, denoted by $\map_1 \sim \map_2$, if $\map_1(v) = \map_2(v)$ for all variables $v$ which are in both $\Dom{\map_1}$ and $\Dom{\map_2}$. If $\map_1 \sim \map_2$, then we write $\map_1 \cup \map_2$ for the mapping obtained  by extending $\map_1$ according to $\map_2$ on all the variables in $\Dom{\mu_2}\setminus\Dom{\mu_1}$.
%We use $f: (\vars \rightarrow \objs) \rightarrow \{ \textsc{true}, \textsc{false} \}$ to denote a function that accepts a mapping and returns true or false.

Given two sets of mappings $\Omega_1$ and $\Omega_2$, the \emph{join}, \emph{union}, \emph{difference} and \emph{left outer join} between $\Omega_1$ and $\Omega_2$ are defined respectively as follows:
\begin{eqnarray*}
\Omega_1 \Join \Omega_2  &=& \{ \mu_1 \cup \mu_2 \mid \mu_1 \in \Omega_1,\, \mu_2 \in \Omega_2 \text{ and } \mu_1 \sim \mu_2 \},\\
\Omega_1 \cup \Omega_2  &=& \{ \mu \mid \mu \in \Omega_1 \text{ or } \mu \in \Omega_2 \},\\
\Omega_1 \setminus \Omega_2  &=& \{ \mu _1 \in \Omega_1 \mid \forall \mu_2 \in \Omega_2 : \mu_1 \sim \mu_2 \text{ does not hold} \},\\
\Omega_1 \LOJ \Omega_2  &=& (\Omega_1 \Join \Omega_2) \cup (\Omega_1 \setminus \Omega_2).
\end{eqnarray*}

With this terminology, a \textit{relational graph pattern} is recursively defined as follows:
\begin{itemize}
\item If $N$ is a navigational graph pattern, then $N$ is also relational graph pattern;
%\item If $R$ is a relational graph pattern and $C$ is a selection condition, then $(R \FILTER C)$ is a relational graph pattern.
\item If $R_1$ and $R_2$ are relational graph patterns, then $(R_1 \AAND R_2)$ and $(R_1 \OPT R_2)$ are relational graph patterns.
\end{itemize}

The evaluation of a relational graph pattern $R$ over a property-domain graph $G$, denoted by $\semp{R}{G}$, is recursively defined as follows:
\begin{itemize}
\item if $R$ is a navigational graph pattern $N$, then $\semp{R}{G} = \semp{N}{G}$;
\item if $R$ is $(R_1 \AAND R_2)$ then $\semp{R}{G} = \semp{R_1}{G} \Join \semp{R_2}{G}$;
\item if $R$ is  $(R_1 \OPT R_2)$ then $\semp{R}{G} = \semp{R_1}{G} \LOJ \semp{R_2}{G}$.
%\item if $R$ is  $(R_1 \FILTER C)$ then 
%  \begin{eqnarray*}
%    \semp{R}{G} &=& \{ \mu \mid \mu \in \semp{R_1}{G} \text{ and } \mu \models C \}
%  \end{eqnarray*}
\end{itemize}

%-----------
\textbf{Selection conditions.}
In addition to match a graph pattern against a property-domain graph, we would like to filter the solutions by imposing selection conditions over the resulting objects (i.e. nodes and edges) and their properties.   
In this sense, a \emph{selection condition} is defined recursively as follows: 
(a) if $v_1, v_2 \in \vars$ and $o \in \objs$, $k_1, k_2 \in \keys$, $v \in \values$ then $(v_1 = v_2)$, $(v_1 = o)$, $v_1.k_1 = v_2.k_2$ and $v_1.k_1 = v$ are selection conditions; and (b) if $C_1, C_2$ are selection conditions, then $(\neg\ C_1)$, $(C_1 \land C_2)$, $(C_1
\lor C_2)$ are selection conditions.

Given a property-domain graph $G=(O,\gamma,\lab,\prop)$, a mapping $\mu$, and a selection condition $C$, we say that $\mu$ satisfies $C$ under $G$, denoted by $\mu \models_G C$, if
\begin{itemize}
\item
$C$ is $({v_1} = {v_2})$, $v_1, v_2 \in \Dom{\mu}$ and $\mu(v_1) = \mu(v_2)$;

\item
$C$ is $({v_1} = o_1)$, $v_1 \in \Dom{\mu}$ and $\mu(v_1) = o_1$;

\item
$C$ is $({v_1.k_1} = {v_2.k_2})$, $v_1, v_2 \in \Dom{\mu}$, 
$\prop(\mu(v_1),k_1) = \prop(\mu(v_2),k_2)$;

\item
$C$ is $({v_1.k_1} = {v})$, $v_1 \in \Dom{\mu}$ and $\prop(\mu(v_1),k_1) = v$;

\item
$C$ is $(\neg C_1)$, and it is not the case that $\mu \models_G C_1$;

\item
$C$ is $(C_1 \land C_2)$, $\mu \models_G C_1$ and $\mu \models_G C_2$;

\item
$C$ is $(C_1 \lor C_2)$, $\mu \models_G C_1$ or $\mu \models_G C_2$.
\end{itemize}

%-----------
\textbf{Solution modifiers.}
We consider an initial set of solution modifiers that allow for applying a final transformation on the solutions generated by a graph pattern. 
These include:
\textsf{selection}, which defines a set of elements (variables and properties) to be returned;
\textsf{order by}, which orders the solutions according to a sort criteria; and
\textsf{limit}, which returns the first $n$ mappings in a sequence of solutions.

%Given a sequence of selection mappings $S$, we have that  $\dom(S) = \bigcup_{\tau \in S} \dom(\tau)$.
%Additionally, given a string $e \in \dom(S)$, we will use $S{\uparrow}e$ to denote that the selection mappings in $S$ satisfy an ascending order with respect to $e$. Similarly, we will use $S{\downarrow}e$ to denote that $S$ satisfies a descending order. 

Let $\mathbf{S}$ be the set of strings, $v \in var$ and $k \in \keys$.
A \emph{selection mapping} is a function $\tau : \mathbf{S} \to \objs \cup \values$.
A \emph{selection element} is either a variable $v$ or an expression $v.k$.   
Assume that there is a simple way to transform a selection element into a string in $\mathbf{S}$.  
Given a sequence of selection mappings $S$ and an integer $n$, the function $\texttt{limit}(S,n)$ returns the first $n$ elements of $S$ when $n > 0$, and returns $S$ otherwise.  

Given a property-domain graph $G=(O,\gamma,\lab,\prop)$, a mapping $\mu$, and a sequence of selection elements $E$, the function $\texttt{sel}(\mu,E)_G$ returns a selection mapping $\tau$ defined as follows:
if $v \in E$ then $``v" \in \dom(\tau)$ and $\tau(``v") = \mu(v)$;
if $v.k \in E$ then $``v.k" \in \dom(\tau)$ and $\tau(``v.k") = \prop(\mu(v),k)$. 
Moreover, given a set of solution mappings $\Omega$, the function $\texttt{select}$ returns a set of selection mappings defined as 
$\texttt{select}(\Omega,E)_G = \{ \texttt{sel}(\mu,E)_G \mid \mu \in \Omega \}$. 

An \emph{order modifier} is a tuple $(e,\beta)$ where $e$ is a selection element and $\beta$ is either \texttt{asc} or \texttt{desc}.
Given a sequence of selection mappings $S$ and an order modifier $o = (e,\beta)$, we say that $S$ satisfies $o$, denoted $S \models o$, if it applies that: 
(i) $\beta$ is \texttt{asc} and $S$ satisfies an ascending order with respect to $e$;
or (ii) $\beta$ is \texttt{desc} and $S$ satisfies a descending order with respect to $e$.  
Moreover, given a sequence of order modifiers $O = (o_1, \dots, o_n)$, we say that $S$ satisfies $O$, denoted $S \models O$, if it applies that:
(i)  $S \models o_1$ when $n = 1$; or
(ii) $S \models o_1$ and, for every sub-sequence of selection mappings $S' \subseteq S$ it applies that $S' \models (o_2, \dots, o_n)$ such that $\tau_i(e_1) = \tau_j(e_1)$ for any pair of selection mappings $\tau_i, \tau_j \in S'$, with $o_1 = (e_1,\beta_1)$.  

%-----------
\textbf{Graph Query.}
A \textit{graph query} $Q$ is defined as a tuple ($R$, $C$, $E$, $O$, $n$), where $R$ is a relational graph pattern, $C$ is a selection condition, $E$ is a sequence of selection elements, $O = \{ o_1, \dots, o_n \}$ is a sequence of order modifiers, and $n$ is a positive integer. We assume that $R$ is the unique mandatory component. 
Given a variable $v \in \dom(R)$, the rest of components have the following expressions by default: $C$ is $v = v$, $E$ is $v$, $O$ is $(v,\texttt{asc})$ and $n = 0$. 

The evaluation of $Q$ over $G$ is defined as $\texttt{limit}(S,n)$ where   
$S = \texttt{Select}(\Omega,E)_G$,  $S \models O$, and 
$\Omega = \{ \mu_{|_V} \mid \mu \in \semp{R}{G} \land \mu \models^G C \}$.

We will assume that every graph query $Q$ = ($R$, $C$, $E$, $O$, $n$) satisfies the following two conditions:
(i)  For every sub-pattern $R' = (R_1 \OPT R_2)$ of $R$ and for every variable $v$ occurring in $R$, it applies that, if $v$ occurs both inside $R_2$ and outside $R'$, then it also occurs in $R_1$;
(ii) It applies that $\var(C) \subseteq \var(R)$.
Then, we say that $Q$ is a \emph{well-designed graph query}.

It is easy to see that a declarative query expression 
\textbf{SELECT} $E$
\textbf{MATCH} $R$
\textbf{WHERE} $C$
\textbf{LIMIT} $n$
\textbf{ORDER BY} $O$, can be transformed into a graph query 
($R$, $C$, $E$, $O$, $n$).

  
%$$
%\begin{array}{ccl}
%\sigma_f(\mset) & = & \{ \mu \in \mset \mid f(\mu) = \textsc{true} \} \\
%\pi_\mathcal{X}(\mset) & = & \{ \mu_{|\mathcal{X}} \mid \mu \in \mset \} \\
%\mset_1 \Join \mset_2 & = & \{\map_1 \cup \map_2 \mid \map_1 \in \mset_1,  \map_2 \in \mset_2, 
% \text{ and } \map_1 \sim \map_2\} \\
%\mset_1 \cup \mset_2 & = & \{\map \mid \map \in \mset_1\text{ or } \map \in \mset_2 \} \\
%%\mset_1 \cup \mset_2 & = & \{\map \mid \map \in \mset_1 \text{ or } \map \in \mset_2\}, \\
%\mset_1 \setminus \mset_2 & = & \{\map_1 \mid \map_1 \in \mset_1 \text{ and } \forall \map_2 \in \mset_2, \map_1 \nsim \map_2\}\%\
%\mset_1 \LOJ \mset_2 & = & (\mset_1 \Join \mset_2) \cup (\mset_1 \setminus \mset_2)
%\end{array}
%$$

%Additional relational operators -- such as aggregation, renaming, binding, etc., -- can be defined and included analogously.

%\ah{TODO: example}

%\ah{TODO: bag semantics}




%%%%%%%%%%%%%%%%%THIS GOES TO THE APPENDIX%%%%%%%%%%


\begin{comment}

\subsection{Concrete syntax}

The language supported by MillenniumDB borrows syntax from popular graph query languages SPARQL \cite{HarrisS13} and Cypher \cite{FrancisGGLLMPRS18}. The following is an example of a query in MillenniumDB which finds all people that a person named John knows, and additionally, the city where these people live, if this information is known:

\begin{lstlisting}
SELECT ?y, ?z
MATCH (?x :Person)-[:knows]->(?y :Person)
	OPTIONAL {(?y)-[:livesIn]->(?z :City)}
WHERE ?x.name == "John"
\end{lstlisting}

Intuitively, the \texttt{SELECT} clause specifies which of the matched variables will be returned (\textit{projection}), while the \texttt{MATCH} clause specifies the basic or navigational graph pattern which we will look for in our graph. We can transform or combine the results of one or more \texttt{MATCH} clauses using relational operators to generate a complex graph pattern. In the example, the \texttt{OPTIONAL} pattern invokes a left-outer-join that extends the obtained result with the name of the city only if this information is known (and assigns no value to \texttt{?z} otherwise). Note that \texttt{OPTIONAL} can be interpreted as \texttt{OPTIONAL MATCH}, i.e., it is a binary operator that combines the results of two basic or navigational graph patterns. Finally, the \texttt{WHERE} clause is used to filter result based on a selection, usually by restricting the values of some of the attributes of a matched object.
  
\begin{figure}
\begin{center}
\begin{lstlisting}
SELECT SelOptions
MATCH  MatchPattern
WHERE  Condition
\end{lstlisting}
\end{center}
\caption{Shape of a query in MillenniumDB}
\label{fig-shape}
\end{figure}

\begin{figure*}
\begin{center}
\fbox{Query elements}
\end{center}
\begin{align*} 
\texttt{SelOptions} & :- \ \textcolor{blue}{\texttt{*}} \ | \ v \ | \ v\textcolor{blue}{\textbf{.}}k \ \quad , \quad v\in \vars, k \in \keys\\
\texttt{MatchPattern} & :- \ \texttt{GraphPattern}\ |\   \textcolor{red}{\texttt{(}}\ \texttt{MatchPattern}\ \textcolor{red}{\texttt{)}} \ \textcolor{blue}{\texttt{OPTIONAL}} \ \textcolor{blue}{\texttt{\{}} \ \texttt{MatchPattern} \ \textcolor{blue}{\texttt{\}}}\\ 
\texttt{GraphPattern} & :- \ \texttt{GraphElement} \ | \  \texttt{GraphElement} \textcolor{blue}{\texttt{\textbf{,}}} \  \textcolor{red}{\texttt{(}} \ \texttt{GraphPattern} \ \textcolor{red}{\texttt{)}}\\
\texttt{GraphElement} & :- \ \texttt{NodePattern} \ |\ \texttt{EdgePattern} \ |\ \texttt{PropertyPath} \\
\texttt{Condition} & :- \ \texttt{Comparison} \ | \ \textcolor{blue}{\texttt{(}}\texttt{Condition \textcolor{blue}{AND} Condition}\textcolor{blue}{\texttt{)}} \ | \  \textcolor{blue}{\texttt{(}}\texttt{Condition \textcolor{blue}{OR} Condition}\textcolor{blue}{\texttt{)}}\\
\texttt{Comparison} & :- \ v\textcolor{blue}{\textbf{.}}k \sim val \ | \ v\textcolor{blue}{\textbf{.}}k \sim v'\textcolor{blue}{\textbf{.}}k' \quad , \quad v, v'\in \vars, k, k'\in \keys, val \in \values, \sim \in \{\textcolor{blue}{\texttt{==,<=,>=,<,>}}\}
\end{align*}
%% I prefer the version below, but it's a pain to formalize
%\begin{align*} 
%\texttt{SelOptions} & :- \ \textcolor{blue}{*} \ | \ v \ | \ v\textcolor{blue}{\textbf{.}}k \ \quad , \quad v\in \vars, k \in \keys\\
%\texttt{BasePattern} & :- \ (\texttt{NodePattern} \ |\ \texttt{EdgePattern} \ |\ \texttt{PropertyPath}) \ | \ (\texttt{NodePattern} \ |\ \texttt{EdgePattern} \ | \ \texttt{PropertyPath})\textcolor{blue}{\textbf{,}} \ \texttt{BasePattern}\\
%\texttt{OptPattern} & :- \ \textcolor{blue}{\{}\texttt{BasePattern}\ (\texttt{\textcolor{blue}{OPTIONAL} OptPatter})?\textcolor{blue}{\}}\\
%\texttt{Condition} & :- \ \texttt{Comparison} \ | \ \textcolor{blue}{(}\texttt{Comparison \textcolor{blue}{AND} Comparison}\textcolor{blue}{)} \ | \  \textcolor{blue}{(}\texttt{Comparison \textcolor{blue}{OR} Comparison}\textcolor{blue}{)}\\
%\texttt{Comparison} & :- \ v\textcolor{blue}{\textbf{.}}k \sim val \quad , \quad v\in \vars, k\in \keys, val \in \values, \sim \in \{\textcolor{blue}{==,<=,>=,<,>}\}
%\end{align*}

\begin{center}
\fbox{Nodes, edges and property paths}
\end{center}
\begin{align*} 
\texttt{NodePattern} & :- \ \textcolor{blue}{\texttt{(}} \ \texttt{Node}? \ \texttt{Labels}? \ \texttt{Properties}? \ \textcolor{blue}{\texttt{)}}\\
\texttt{Node} & :- \ v \in \vars \ | \ o\in \objs\\
\texttt{Labels} & :- \ \textcolor{blue}{\textbf{:}}l \ | \ \textcolor{blue}{\textbf{:}}l \ \texttt{Labels} \quad , \quad l\in \labels\\
\texttt{Properties} & :- \ \textcolor{blue}{\texttt{\{}} \ \texttt{PropertyList} \ \textcolor{blue}{\texttt{\}}}\\
\texttt{PropertyList} & :- \ k\textcolor{blue}{\textbf{:}}val \ | \ k\textcolor{blue}{\textbf{:}}val\textcolor{blue}{\textbf{,}}\ \texttt{PropertyList}  \quad , \quad k\in \keys, val\in \values\\
 & \\
 \texttt{EdgePattern} & :- \ \texttt{NodePattern} \ \texttt{\textcolor{blue}{-}} \texttt{Edge}? \texttt{\textcolor{blue}{>}} \ \texttt{NodePattern} \ |\            \texttt{NodePattern} \ \texttt{\textcolor{blue}{<-}} \texttt{Edge}? \texttt{\textcolor{blue}{}} \ \texttt{NodePattern} \\
\texttt{Edge} & :- \ \texttt{\textcolor{blue}{[}} \ v? \ \texttt{Type}? \ \texttt{Properties}? \ \texttt{\textcolor{blue}{]-}} \quad , \quad v\in \vars \\
 \texttt{Type} & :-\ \textcolor{blue}{\textbf{:}}o \ | \ \textcolor{blue}{\texttt{=TYPE(}}v\textcolor{blue}{\texttt{)}} \quad , \quad o\in \objs, \ v\in \vars\\
 & \\
 \texttt{PropertyPath} & :- \ \texttt{NodePattern} \ \textcolor{blue}{\texttt{=[}} \ \texttt{pathExp} \ \textcolor{blue}{\texttt{]=>}} \ \texttt{NodePattern} \ |\  \texttt{NodePattern} \ \textcolor{blue}{\texttt{<=}} \textcolor{blue}{[} \ \texttt{pathExp} \ \textcolor{blue}{\texttt{]=}} \ \texttt{NodePattern}\\
% \texttt{PropertyPath} & :- \ \texttt{NodePattern} \ (\textcolor{blue}{=[} \texttt{PathVar}? \ \texttt{pathExp} \textcolor{blue}{]})? \textcolor{blue}{=>} \ \texttt{NodePattern} \ |\ \\
% & \quad \quad \texttt{NodePattern} \ \textcolor{blue}{<=} (\textcolor{blue}{[} \texttt{PathVar}? \ \texttt{pathExp} \textcolor{blue}{]=})? \ \texttt{NodePattern}\\
 \texttt{pathExp} & :- \ \texttt{\textcolor{blue}{\textbf{:}}}o  \ |\ \textcolor{blue}{\hat{ }} \ \texttt{pathExp} \ |\  \textcolor{blue}{\texttt{(}}\texttt{pathExp\textcolor{blue}{\textbf{/}}pathExp}\textcolor{blue}{\texttt{)}} \ |\ \texttt{pathExp}^{\textcolor{blue}{\texttt{*}}} \ |\\
 & \quad \quad \texttt{pathExp}^{\textcolor{blue}{\texttt{+}}} \ | \  \texttt{pathExp\textcolor{blue}{\{}n\textcolor{blue}{\textbf{,}}m\textcolor{blue}{\}}} \ |\ \textcolor{blue}{\texttt{(}}\texttt{pathExp \textcolor{blue}{|} pathExp}\textcolor{blue}{\texttt{)}} \ |\ \texttt{pathExp}\textcolor{blue}{\texttt{?}} \quad , \quad o\in \objs, \texttt{n,m}\in \mathbf{N}, \texttt{n}\leq \texttt{m}
\end{align*}
\caption{Specification of query patterns in MilleniumDB. Blue symbols are taken literally. Red brackets in \texttt{MatchPattern} and \texttt{GraphPattern} are grouping specification for unambiguous parsing, and are not specified when writing the query.}
\label{fig-syntax}
\end{figure*}

The general structure of a query in MillenniumDB is defined in Figure \ref{fig-shape}. The syntax of different patters that appear in a query is defined in Figure \ref{fig-syntax}. The workhorse of a query in MillenniumDB is specified in the \texttt{MatchPattern}, which specifies a pattern that needs to be present in our graph. The \texttt{Condition} from the \texttt{WHERE} clause is then applied as a filter to the selected results, and \texttt{SelOptions} specify which data is to be projected out as the final result. To illustrate the use of these components consider following query:

\begin{lstlisting}
SELECT *
MATCH (?x :Person), (?y)-[:knows]->(?z), (?y)=[:follows*]=>(?w)
	OPTIONAL {(?x)-[:knows]->(?w)}
		OPTIONAL {(?x)-[:follows]->(?w)}
WHERE ?x.name == ?y.name
\end{lstlisting}

As specified by Figure \ref{fig-syntax}, the \texttt{MatchPattern} consists of a single \texttt{GraphPattern}, followed by a series of \texttt{OPTIONAL} patterns. The \texttt{GraphPattern} is a series of \texttt{GraphElements} which match a specific node, edge, or a path between nodes, separated by a comma. In the example above, the pattern \texttt{(?x :Person)} is saying that 
 we want to match a node with the label \texttt{Person}, and store the result in the variable \texttt{?x}. Similarly, \texttt{(?y)-[:knows]->(?z)} matches an edge between a node stored in the variable \texttt{?y} and a node stored in the variable \texttt{?z}, that has a type \texttt{knows}. Lastly, the pattern \texttt{(?y)=[:follows*]=>(?w)} looks for a pair of nodes, stored in \texttt{?y} and \texttt{?w}, respectively, connected by a path of arbitrary length, where each edge has the type \texttt{follows}. Intuitively, the result of a \texttt{GraphPattern} can be thought as obtained by joining the results of each of its constituent \texttt{GraphElements}.
 
 Following a \texttt{GraphPattern}, we have a series of \texttt{OPTIONAL} statements. Each of these can again specify a new \{\ \texttt{MatchPattern}\ \}, placed inside braces, and can thus include nested \texttt{OPTIONAL} statements. Several consecutive \texttt{OPTIONAL} statements are parsed as being grouped to the left. We signal this in Figure \ref{fig-syntax} by placing the \texttt{MatchPattern} to the left of an optional into red braces. Similarly, in order to parse them unambiguously, \texttt{GraphPatterns} can be thought as being grouped to the right. That is, the \texttt{MatchPattern} above is grouped as follows:
 
\begin{lstlisting}
( ( (?x :Person), (?y)-[:knows]->(?z), (?y)=[:follows*]=>(?w) )
	OPTIONAL { (?x)-[:knows]->(?w) } )
		OPTIONAL { (?x)-[:follows]->(?w) }
\end{lstlisting} 
 

The semantics of a query $q$ over a property-domain graph $G$ is defined in terms of mappings, analogously to SPARQL \cite{PerezAG09}, or to homomorphism based semantics of property graphs \cite{AnglesABHRV17}. A \textit{mapping} is a partial function $\mu: \vars \mapsto \objs$. The \emph{domain} $\Dom{\map}$ of a mapping $\map$ 
is the set of variables on which $\map$ is defined. Additionally, we will assume that $\mu(o)=o$, for all $o\in \objs$. We begin by defining the semantics of mappings over each atomic block of a query, that is over a \texttt{NodePattern, EdgePattern} and \texttt{PropertyPath}. Before doing this, notice that each \texttt{NodePattern} can have an explicit identifier (e.g. in \texttt{(Q320 :Person)}), or a variable (e.g. in \texttt{(?x :Person)}), and each \texttt{Edge} can have a variable (e.g. in \texttt{(?x)-[?e :knows]->(?y)}). When these are not present, they are assumed to be existentially quantified; namely, when we write \texttt{(Q320)-[:knows]->()}, we are simply trying to count all the nodes that \texttt{Q320} can reach via an edge of the type \texttt{knows}, and these are ``virtually" assigned to an ``invisible" variable \texttt{?y} inside the empty node pattern\texttt{()}. 

When defining the set of variables used in a query $q$, without loss of generality, we will assume that all \texttt{NodePattern} or \texttt{Edge} elements which do not have either an explicit identifier, nor a variable, are assigned a unique fresh variable not used elsewhere in $q$. We call such variables \textit{anonymous variables} of $q$, and denote them $\avar{q}$. All the \textit{explicit variables} of a query $q$, that is, the ones appearing in the definition of $q$, are denoted by $\evar{q}$. The set of variables of $q$, denoted $\qvars{q}$ equals the union $\avar{q} \cup \evar{q}$. We can now define the semantics of  a query $q$ over a property domain-graph $G=(O,\gamma,\texttt{lab},\texttt{prop})$, denoted $\semp{q}{G}$, inductively as the set of all mappings $\mu:\qvars{q}\mapsto \objs$.

Basically, we do this in the next section in a bit more general setting (optional patterns are more general there).

\riveros{Can we query the domain graph, namely, the `keys' in the function? Also I would write some queries using the running example of Section 2.} 

%\begin{itemize}
%\item If $q$ \texttt{:- (id :l$_1\cdots$:l$_m$) \{k$_1$:v$_1,\ldots ,$k$_n$:v$_n$\})}, with \texttt{id} being either a variable, or $o\in \objs$, is a \texttt{NodePattern}, then the set  $\semp{q}{G}$ contains all mappings $\mu:\qvars{q}\mapsto \objs$, such that:
%\begin{itemize}
%\item $\mu(\texttt{id})\in O$,
%\item $\{l_1,\ldots, l_m\} \subseteq \lab(\mu(\texttt{id}))$, and
%\item $\prop(\mu(\texttt{id}),k_i) = v_i$, for $i=1\ldots n$.
%\end{itemize}
%Notice that here $\mu = \emptyset$ belongs to $\semp{q}{G}$ whenever \texttt{id} equals an explicit object identifier $o\in \objs$, and the node $o$ has appropriate labels and properties, and is present in the database.
%\item If $q$ \texttt{:- NodePattern1-[ ?x $t$ \{k$_1$:v$_1,\ldots ,$k$_n$:v$_n$\} ]->NodePattern2}, with \texttt{?x} a variable and $t$ either an object, or a type variable, is an \texttt{EdgePattern}, and where \texttt{id1} and \texttt{id2} are identifiers for \texttt{NodePattern1}, and \texttt{NodePattern2}, then $\semp{q}{G}$ contains all mappings $\mu:\qvars{q}\mapsto \objs$ where:
%\begin{itemize}
%\item $\mu_{|\qvars{\texttt{NodePattern1}}} \in \semp{\texttt{NodePattern1}}{G}$,
%\item $\mu_{|\qvars{\texttt{NodePattern2}}} \in \semp{\texttt{NodePattern2}}{G}$,
%\item $\gamma(\mu(\texttt{?x})) = (\mu(\texttt{id1}),\mu(t),\mu(\texttt{id2}))$, and
%\item $\prop(\mu(\texttt{?x}),k_i) = v_i$, for $i=1\ldots n$.
%\end{itemize}
%\item If $q$ \texttt{:- NodePattern1-[ pathExp ]->NodePattern2} is a \texttt{PropertyPath}, with \texttt{id1} and \texttt{id2}  identifiers for \texttt{NodePattern1}, and \texttt{NodePattern2}, then $\semp{q}{G}$ contains all mappings $\mu:\qvars{q}\mapsto \objs$ where:
%\begin{itemize}
%\item $(\mu(\texttt{id1}),\mu(\texttt{id2})) \in \semp{\texttt{pathExp}}{G}$, with $\semp{\texttt{pathExp}}{G}$ as defined in Figure \ref{fig-pathexp}.
%\end{itemize}
%\end{itemize}
%
%
%To combine results of multiple elements of a  \texttt{MatchPattern}, we need to specify how to join mappings and sets of mappings. Two mappings $\map_1$ and $\map_2$ are \emph{compatible} (written as $\map_1 \sim \map_2$) 
%if $\map_1(?x) = \map_2(?x)$ for all variables $?x$ which are in both $\Dom{\map_1}$ and $\Dom{\map_2}$. 
%If $\map_1 \sim \map_2$, then 
%we write $\map_1 \cup \map_2$ for the mapping obtained 
%by extending $\map_1$ according to $\map_2$ on all the variables in $\Dom{\mu_2}\setminus\Dom{\mu_1}$. Given two sets of mappings $\mset_1$ and $\mset_2$, 
%the \emph{join}, \emph{difference} and \emph{left outer join} between $\mset_1$ and $\mset_2$ are defined respectively as follows:
%$$
%\begin{array}{ccl}
%\mset_1 \Join \mset_2 & = & \{\map_1 \cup \map_2 \mid \map_1 \in \mset_1,  \map_2 \in \mset_2, 
% \text{ and } \map_1 \sim \map_2\} \\
%%\mset_1 \cup \mset_2 & = & \{\map \mid \map \in \mset_1 \text{ or } \map \in \mset_2\}, \\
%\mset_1 \setminus \mset_2 & = & \{\map_1 \mid \map_1 \in \mset_1,   \text{ and } \forall \map_2 \in \mset_2, \map_1 \nsim \map_2\}\\
%\mset_1 \LOJ \mset_2 & = & (\mset_1 \Join \mset_2) \cup (\mset_1 \setminus \mset_2)
%
%\end{array}
%$$
%
%With this notation in hand, and with the definition of the semantics of \texttt{GraphElement}, we can complete the definition of \texttt{GraphPattern} and \texttt{MatchPattern} by setting: 
%\begin{itemize}
%\item If $q$ \texttt{:- GraphElement, (GraphPattern)}, then
% $$\semp{q}{G} = \semp{\texttt{GraphElement}}{G} \Join \semp{\texttt{GraphPattern}}{G}$$
%\item If $q$ \texttt{:- ( MatchPattern ) OPTIONAL \{ MatchPattern  \}}, then
% $$\semp{q}{G} = \semp{\texttt{MatchPattern}}{G} \LOJ \semp{\texttt{MatchPattern}}{G}.$$
%\end{itemize}
%
%For an arbitrary query $q$, we can determine all the mappings that satisfy its \texttt{MATCH} clause. NEED TO DO SELECT/PROJECT WITH THE REMAINING CLAUSES!!!!
%
%\bigskip
%
%\bigskip
%
% Namely, let $Var(q)$ be the set of all object variables appearing in $q$. Intuitively, a mapping $\mu : Vars(q)\mapsto \objs$ is a \textit{solution} for $q$ over $G$, if replacing every variable \texttt{?x} in $q$s \texttt{MATCH} clause with $\mu(\texttt{?x})$ results in a patter that is valid in $G$. Formally, we have to define when a pattern is valid in $G$ inductively. For instance, a node pattern \texttt{(?x :Company :TechStartup \{city:"Santiago"\})} is valid in $G$ under a mapping $\mu$, if (i) $\mu(\texttt{?x})\in O$; (ii) $\{\texttt{:Company, :TechStartup}\} \subseteq \lab(\mu(\texttt{?x}))$; and (iii) $\prop(\mu(\texttt{?x}),\texttt{city}) = \texttt{Santiago}$.

%NEED TO DEFINE: deanonymization (put variables in all node/edge patterns that have no var nor fixed id). Call this $AVars(q)$. A mapping needs to go from $Vars(q)\cup AVars(q)$. Then it suffices to define what happens on Node/edge/Property path patterns, and we are done. For optionals it gets a bit tricky due to nesting!!! Still thinking about how to do this with optionals. Perhaps have version 0 without optionals? Just to have a core of the language? I removed path variables from version 0 of the language. We can add them after defining the semantics.






\end{comment}


==> sections/storage.tex <==
The default storage mechanism in MillenniumDB are B+ trees \cite{ramakrishnan00}. For this purpose, we built a B+ tree template for fixed sized records, which allows to guard different property-domain graph elements, and their relationships. 

Internally, all object are represented as 8 byte identifiers. To optimize query execution, identifiers are divided into classes (the first byte of the identifier specifies a class it belongs to). The main classes in a property-domain graph $G=(O,\gamma,\lab,\prop)$ are:
\begin{itemize}
\item Named nodes, which are objects in the domain graph for which an explicit name is available (e.g. Q320 in WikiData).
\item Anonymous nodes, which are internally generated objects without an explicit name available to the user.
\item Edges, which are objects in the domain of $\gamma$, and are always anonymous nodes (recall that the query language does not allow to identify a connection with a concrete object).
\item Inlined values, which are values that fit into 7 bytes of the identifier after the mask (e.g. 7 byte strings, integers, etc.).
\item External values, which are values longer than 7 bytes (e.g. long strings).
\end{itemize}

At this moment, only external value supported is a long string; however, the implementation interface allows to add different value types in a simple manner. All records guarded in B+ trees are composed of identifiers. Therefore, when we write $o\in O$, we are referring to the identifier of the object $o$. We will later explain how explicit names and string values are handled.

The following B+ tree indices are created to store a property-domain graph $G=(O,\gamma,\lab,\prop)$:
\begin{itemize}
\item {\it Nodes}, which contains the identifiers of all the objects present in the database and records of size 1.
\item {\it NodeLabel}, which contains pairs $(o,l)$, where $o\in O$, and $l\in \lab(o)$ is the label. Both permutations of the pair are available by default.
\item {\it ObjectKeyValue}, which contains triples $(o,k,v)$ such that $o\in O$ and $\prop(o,k)=v$. Additionally, a permutation {\it KeyValueObject} is created by default.
\item {\it FromToTypeEdge}, which contains quads $(s,o,p,e)$, such that $\gamma(e) = (s,p,o)$. Additionally, the permutations {\it ToTypeFromEdge}, {\it TypeFromToEdge} and {\it TypeToFromEdge} are created by default.
\riveros{It shouds like we have 4 B+-trees, when we have 7. I would be more explicit on this.}
\end{itemize}

All the B+ trees are created through a bulk-import phase, which loads multiple tuples of sorted data, instead of creating the trees by inserting records one by one.

Notice that in storing connections, we always keep the connection identifier at the end of the tuple. This is because the connection identifier is a key for this relation, so efficient lookups of other components only need to scan the source node, the target node, or the connection type. In order to allow lookups by edge identifier, we also store a table called {\it EdgeTable}, which contains triples of the form $(s,p,o)$, such that the position in the table equals to the identifier of the object $e$ such that $\gamma(e)=(s,p,o)$. This implies that edge identifiers (elements in the domain of $\gamma$) must be assigned consecutive ids starting from zero, and are thus generated by MillenniumDB, and not specified by the user. For this reason, no object identifiers are available in the edge position in the queries in MillenniumDB.

Finally, we need to explain how explicit values (e.g. string names of nodes, their labels, key names, key values, etc.) are stored, and how these are transformed to their internal ids and vice versa. For this, we have a single binary file called {\it ObjectFile}, which contains all of these values concatenated together. In particular, the identifier of such an explicit value will be equal to the position where it is written in the {\it ObjectFile}, thus allowing efficient lookups of a value via its id. The identifiers are generated upon loading, and an additional hash table is kept to map (hash) of a string to its identifier, in order to ensure that no value is inserted twice, and to transform explicit values given in a query to their internal ids upon query execution.

All of the stored relations are accessed through linear iterators which allow accessing the information one tuple at a time. All of the data is stored on pages of fixed (but parametrizable) size (4kB at this point). The data from disc if loaded into a shared main memory buffer, whose size can be specified upon initializing the MillenniumDB server. The buffer uses the standard clock page replacement policy \cite{ramakrishnan00}. Additionally, for improved performance, upon initializing the server, it can be specified that the \textit{ObjectFile} be loaded into main memory in order to quickly convert internal identifiers to string and integer values that do not fit into 7 bytes.

%At this point, the implementation only supports inserts and bulk loading, but no deletion of records.

%\bigskip
%
%Given that $E$ is a key for this relation, using a data structure that permits prefix-lookups (e.g., a B+ tree), the index-order permutations required for efficient evaluation only depend on $SPO$ (and $E$ alone). Index orders on (e.g.,) $SPOE$, $OSPE$, $POSE$ and $ESPO$ allow for looking-up any atomic query pattern; e.g., a pattern such as $Q(?,P,?,\underline{E})$ can be retrieved as $Q(?,?,?,\underline{E})$ on $ESPO$, which will return at most one tuple (whose $P$ we can then check). Additionally, a table that allows searching when $E$ is known is needed, for instance ESPO ($\gamma(e_1) = (Q320,P31,Q466956) $). Note an engine might decide to represent an internal identifier for $E$ as its position in this table (plus some type prefix), thus effectively allowing to drop the first column. \ah{... just importing this text from model; fits better here I think, though the notation of $SPOE$ needs to be introduced.}
